Exploring Self-supervised Logic-enhanced Training for Large Language Models

Existing efforts to improve logical reasoning ability of language models have predominantly relied on supervised fine-tuning, hindering generalization to new domains and/or tasks. The development of Large Langauge Models (LLMs) has demonstrated the capacity of compressing abundant knowledge into a single proxy, enabling them to tackle multiple tasks effectively. Our preliminary experiments, nevertheless, show that LLMs do not show capability on logical reasoning. The performance of LLMs on logical reasoning benchmarks is far behind the existing state-of-the-art baselines. In this paper, we make the first attempt to investigate the feasibility of incorporating logical knowledge through self-supervised post-training, and activating it via in-context learning, which we termed as LogicLLM. Specifically, we devise an auto-regressive objective variant of MERIt and integrate it with two LLM series, i.e., FLAN-T5 and LLaMA, with parameter size ranging from 3 billion to 13 billion. The results on two challenging logical reasoning benchmarks demonstrate the effectiveness of LogicLLM. Besides, we conduct extensive ablation studies to analyze the key factors in designing logic-oriented proxy tasks.

==> backs/0.abstract.tex <==
\begin{abstract}
Recent research progress over Natural Language Processing (NLP) demonstrates a huge impact due to the emergent capability of Large Language Models (LLMs), e.g., PaLM, InstructGPT, LLaMA, ChatGPT, and GPT-4. LLMs can perform very well on various tasks using only several labeled samples as prompt without task-specific fine-tuning. 
Specifically, with the help of Chain-of-Thought (CoT), LLM is also able to conduct multi-step arithmetic reasoning and commonsense reasoning. However, in our preliminary experiments, we find that LLM cannot outperform the much smaller language models with fine-tuning, e.g., RoBERTa-Large, on the logical reasoning tasks. Furthermore, even CoT does not make significant improvements.
To this end, in this paper, we aim to explore the possible reasons why LLMs perform much worse on logical reasoning of text.
Besides, considering the constraints brought by API-based usage and LLMs' sensitivity to prompts and instructions, we also try to provide some insights to future research by exploring if any of previous data-driven approaches can still benefit LLMs with logical reasoning capability. Specifically, we integrated MERIt, a self-supervised pre-trainign approach for logical reasoning, into FLAN-T5-3B, and the results on two challenging logical reasoning benchmarks demonstrate its effectiveness under both fine-tuning and prompting settings.
\end{abstract}

==> backs/1.intro-0521.tex <==

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{image/intro_example_v1_0.pdf}
%     \caption{An instance of logical reasoning from the ReClor dataset. 
%     (i) represents the involved logical variable, e.g., entities or phrases. The reasoning structure is summarized at below.}
%     \label{fig:reclor-example}
%     \vspace{-0.3cm}
% \end{figure}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{image/zs-cot-example-v1-0.pdf}
%     \caption{An example from ReClor dataset illustrating the prompting response under zero-shot and zero-shot CoT settings, respectively.}
%     \label{fig:cot-example}
%     \vspace{-0.3cm}
% \end{figure*}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{image/Dingtalk_20230413185639.jpg}
%     \caption{An example of chain-of-thought prompting in arithmetic reasoning (math word problem solving.}
%     \label{fig:cot-math-example}
%     \vspace{-0.3cm}
% \end{figure}


\section{Introduction}
\label{sec:intro}
\input{tables/preliminary}

\ding{missing citations for some papers like Lets think step by step}\\
\ding{no figures or data visualization. Very content heavy and very dry for reviewers. Need to work on the presentation after the arxiv deadline}\\
\ding{Not enough insights. Should think about how to make the analysis more attractive and interesting after arxiv deadline}\\
\ding{The second question is not very clear. can the
introduced logic knowledge be generalized to hy-
brid tasks? What does hybrid task mean? Refine after arxiv deadline}


% \ding{The whole Intro needs to rewrite. It sounds like an evaluation only. Need to have a good story to convince the reviewers. The paper title is also too plain. You need a good title to attract attention.}

% \ding{A proposed storyline for the paper: 1. Talk about the progress of logical reasoning in NLP. Why logical reasoning is important and what were the methods? 2. LLMs have pushed the performance of  reasoning, can include numerical reasoning, xxx reasoning. You can mention related works like PAL, etc. Talk about how they differentiate with the traditional methods. 3. However, there is a lack of systematic evaluation of logical reasoning / LLMs are still weak in logical reasoning. 4. What is missing / What is the gap to be closed? Why is it important to do so? 5. Mention what you have done and your insights and contribution briefly.}


% \ding{Here are a few possible paraphrased versions of the paper title to make it more attention-grabbing:$
% "Why Logic-enhanced Training is a Game-Changer for Large Language Models"
% "Revolutionizing Language Models: The Crucial Role of Logic-enhanced Training"
% "Unleashing the Full Potential of Language Models with Logic-enhanced Training"
% "Logic + Language: The Winning Combination for Next-gen AI Training"
% "Breaking Barriers: How Logic-enhanced Training Takes Language Models to New Heights"
% "Why Logic-enhanced Training is Critical for Empowering Large Language Models"
% "Unleashing the Full Potential of Language Models with Logic-enhanced Training"
% "Revolutionizing Language Learning: The Importance of Logic-enhanced Training for Large Language Models"
% "Going Beyond Traditional Methods: How Logic-enhanced Training Improves Large Language Models"
% "The Logic Revolution: Why Large Language Models Need Logic-enhanced Training to Succeed"
% "Mastering Language: Enhancing Large Language Models with Logic-based Training"
% "Logic Meets Language: The Game-changing Approach to Training Large Language Models"
% "From Good to Great: How Logic-enhanced Training Takes Large Language Models to the Next Level"
% "Transforming Language Understanding with Logic-enhanced Training for Large Language Models"
% "Breaking the Limits: The Necessity of Logic-enhanced Training for Large Language Models".$}

% Version v1.0
% Logical reasoning has long been treated as a complex ability beyond fundamental natural language understanding, 
% % and also serves as the foundation to perform decision making and planning \teng{Any References?}. 
% and also serves as an essential foundation in negotiation, debate and writing \textit{etc}~\citep{reclor}. 
% Since the widely explored paradigm of fine-tuning after pre-training, it has been realized that the logic prior can hardly be learned from label-free data  through vanilla language modeling~\citep{rulebert,clark2021transformers,lm-cannot-plan}.
% % \teng{Any References show this conclusion?}. 
% Motivated from this, a certain amount studies have explored the data-driven method through data augmentation \citep{lreasoner,merit} as well as synthesis \citep{clark2021transformers}, or building neural-symbolic systems \citep{ar-lsat}, to enhance the logical reasoning ability of deep neural networks. 
% Though some of these approaches have reached or even outperformed the human performance on standard logical reasoning benchmarks via fine-tuning pre-trained language models using supervised data, the generalization ability of the trained models for domains and tasks is hindered. 
%
% On the other hand, when scaled up to extreme size, the causal language models turn to become zero-shot or few-shot learners. The required abilities can be activated via human instructions or few-shot in-context exemplars, making the large language models (LLMs) to easily deal with different tasks without changing parameters. However, when evaluated on logical reasoning benchmarks, as shown in Table~\ref{tab:pre-exp}, the LLM, i.e., ChatGPT\footnote{https://openai.com/blog/chatgpt}, falls far behind the fine-tuned much smaller models. And the one augmented with Chain-of-Thought~\citep{chain-of-thought} also cannot make significant improvements. Besides, we also conducted few-shot experiments under both answer-only and auto-generated CoT setting. The limited improvements compared with zero-shot baseline also suggest that LLMs fail to parse the latent reasoning structure and apply to new problems. All of the preliminary experimental results have demonstrated that the absence of logic can be nature of causal language modeling, and hardly be addressed by scaling up.

% Version v2.0
Logical reasoning has long been treated as a complex ability beyond fundamental natural language understanding, and also serves as an essential foundation in negotiation, debate and writing~\citep{reclor}. 
Extensive efforts have been made to enhance logical reasoning ability of language models. However, fine-tuning based approach requires reasonable amount of annotated training data, and hinders the model to generalize to new tasks due to the mismatch of data distribution and optimization objective.
% , e.g., fine-tuning on multiple choice question answering and predicting on natural language inference task. 
On the other hand, the recent development of Large Language Models (LLMs), e.g., PaLM~\citep{palm}, LLAMA\citep{touvron2023llama}, ChatGPT\footnote{https://openai.com/blog/chatgpt}, GPT-4\footnote{https://openai.com/product/gpt-4}, and Bard\footnote{https://bard.google.com/}, suggests that LLMs can serve as a proxy to compress abundant knowledge, and solve various tasks following human instructions with less  specialization. However, as shown in Table \ref{tab:pre-exp}, our preliminary experiments on logical reasoning benchmarks reveal that LLMs also lack the ability about logical reasoning. There are also results showing that the promotion brought by few-shot exemplars or Chain-of-Thought (CoT) prompting \citep{chain-of-thought} is also limited.

As demonstrated by the evaluations on various benchmarks~\citep{qin2023chatgpt-eval,bang2023chatgpt-eval,wang2023gcre-gpt,mt-chatgpt2023}, logic is not the only knowledge that LLMs are short of, e.g., arithmetic reasoning and knowledge grounding.
In order to mitigate the absence of specific complex capability and avoid using too much annotated data, some work tends to employ external tools, or calling predefined API, such as search engine (information retriever)~\citep{toolformer,arm-survey-lecun}, SQL query~\citep{binder2022cheng}, or calculator~\citep{pal2022gao,pot2022chen}. 
The advantage is that the external tools or APIs can provide accurate results with explicable execution steps, and decouple the complex inference process with semantic understanding and parsing, which the LLMs are more capable on.
% Though promising, similar methodology can be circumscribed when applied to logical reasoning. The tool-based hybrid system requires both finite operation space and execution steps, e.g., the scenarios where the premises are translated from first-order logic or symbolic systems. 
Though promising, similar methodology can be circumscribed when applied to logical reasoning of text. The tool-based hybrid system requires both well-defined executor and explicit arguments. For example, it can be more suitable for the first-order logic presented with formal language and symbols.
However, in natural language based logical reasoning, the logical variables could be arbitrary entities and phrases, leading to extreme difficulty in building executable symbolic logical reasoners. 
% \teng{this paragraph can be kept}

% To this end, in this paper, we aim to explore if the logic-enhanced training could help introduce logic prior into LLMs and keep the generalization as much as possible. 
% To this end, in this paper, we aim to explore logic-enhanced training for LLMs and keep the generalization as much as possible.
In this paper, we aim to explore the logic-enhanced training for LLMs.
% Nevertheless, most methods focusing on data augmentation or synthesis~\citep{lreasoner} have significant mismatch on training objectives with causal language modeling, \jiao{I need two motivations here.}, and may cause the degradation of in-context learning.
% To tackle the above problems, we proposed a auto-regressive version of MERIt~\citep{merit}, a self-supervised pre-training method for logical reasoning, which is originally designed as contrastive learning.
Recent work activating the potential ability of LLMs mostly rely on supervised instruction tuning\footnote{In this paper, we use \textit{supervised fine-tuning} to refer the training process rely on labels annotated by human and LLMs. \textit{Self-supervised} training is also supervised learning but the labels are constructed from natural data.}~\citep{instructgpt}. Through either template-based task-specific data~\citep{aribandi2022ext5,flan,flan-v2,zeroprompt,sanh2022multitask-t0} or open-domain instruction-response pairs~\citep{self-instruct2022wang,wizardlm2023xu}, they all rely on high quality annotations from human expert or teacher LLMs, leading to high difficulty and cost in collecting logic-specific data.
In order to alleviate the data sparsity, we propose to post-train LLMs via self-supervised objectives. Specifically, we introduce MERIt~\cite{merit}, a self-supervised pre-training method for logical reasoning, which was originally designed as contrastive learning. We have explored both the original framework and the auto-regressive variant to seek the trade-off between computation overhead and the benefits.
% \teng{Besides, the data for MERIt training is constructed from Wikipedia, which can help avoid the over-fitting to specific domain: do not need?}. 
We test the performance based on FLAN-T5~\citep{flan-v2} and LLaMA~\citep{touvron2023llama}, with model sizes ranging from 3 billion to 13 billion to verify its scabalility. 


% The experimental results on two logical reasoning benchmark demonstrates the effectiveness of our proposed method.
% and verified the feasibility and necessity of logic-enhanced training for LLMs. 
% Besides, the improvements under in-context learning also suggest the feasibility to augment complex ability of LLMs without supervised fine-tuning.
% Finally, we have discussed the possible factors relevant to logic prior in raw text corpus and the weakness of current LLMs on logical reasoning.
Our experiments study two questions: (1) is it possible to enhance logic ability without task-specific fine-tuning for LLMs? And (2) can the introduced logic knowledge be generalized to hybrid tasks?
For the first question, we find that the LLMs post-trained with MERIt objective can perform better on logical reasoning benchmarks without fine-tuning on them. Particular, LLaMA-based models can achieve better accuracy without open-domain instruction tuning.
As the second question, we find that the learned logic ability can also boost the performance on general reasoning tasks, i.e., DREAM~\citep{dream} and BIG-Bench-Hard~\citep{big-bench-hard}.
In a nutshell, the contribution of this paper can be summarized as follows:
\begin{enumerate}
    \item We evaluate the capability of LLMs on logical reasoning benchmarks, demonstrating weakness of LLMs on performing logical reasoning.
    \item We successfully integrate MERIt with LLMs, demonstrating the feasibility to introduce complex ability into LLMs without task-specific fine-tuning.
    % \item To bring more insights to the community, we try to introduce the data-driven approach into existing LLMs, and verified its effectiveness under both fine-tuning and in-context learning settings.
    \item We have conducted extensive experiments on both FLAN-T5 and LLaMA series, with model parameter size ranging from 3 billion to 13 billion. The results on logical reasoning and symbolic reasoning benchmarks demonstrate the effectiveness of our approach. We have also explored the possible effects of different pre-training strategy to bring some insights to future research.
\end{enumerate}
% \teng{still need more polishing, i will do another round probably on 11-May-2023.}

% ===================================

% In the past few months, the released Large Language Models (LLMs), e.g., PaLM~\citep{palm}, \ding{LLAMA\citep{touvron2023llama}}, ChatGPT\footnote{https://openai.com/blog/chatgpt}, GPT-4\footnote{https://openai.com/product/gpt-4}, and Bard\footnote{https://bard.google.com/}, have surprised public greatly with fluently chatting, abundant world knowledge, strong ability of human assistance, as well as emergent complex capabilities such as arithmetic reasoning, commonsense reasoning, and logic. \teng{Todo by teng: remove and logic}. 
% However, considering the closed source of most of these largest models, systematic evaluation from different perspectives was once absent. Motivated by this, some recent studies have conducted series analysis over a wide range of NLP tasks~\citep{qin2023chatgpt-eval,bang2023chatgpt-eval,wang2023gcre-gpt,mt-chatgpt2023}, and the experimental results have revealed the gap between LLMs and previous state-of-the-art methods. 
% Yet, for logical reasoning, most experiments focus on either simple discrete operations~\citep{qin2023chatgpt-eval} or those built on formal language~\citep{bang2023chatgpt-eval}, which is transformed from first-order logics via template based method.
% \teng{todo by teng: too fast here, we need slow down a little bit.  }
% % Yet, the logical ability of LLMs is still unexplored.  
% Another category of logical reasoning problem is coupled with natural language, where the logical variables are often phrases, and can be difficult to be parsed into strict logic form. And it requires the understanding of natural language predicates, instead of logic operator.
% \teng{todo by teng: maybe we need an example}

% \ding{Need to mention works like PAL. They are good at numerical reasoning but doesn't apply to logical reasoning}

% In order to complete the evaluation of LLMs \teng{todo by teng: maybe we do not need to write from the perspective of evaluation, we can highlight the logic-enhanced pretrained}, we first conducted experiments on two natural language logical reasoning benchmarks, i.e., LogiQA-v2~\citep{logiqa} and ReClor~\citep{reclor} with zero-shot prompting and zero-shot Chain-of-Thought (CoT) prompting. \teng{why these two datasets? Say the reason} 

% As shown in Table~\ref{tab:pre-exp}, we can conclude that LLMs still perform much worse than the fine-tuned much smaller models on logical reasoning. \teng{todo by Jiao: we need to move this table into experiments, we do not need this table here, just say the conclusion in the same way as abstract}
% Furthermore, utilizing zero-shot CoT, i.e., \teng{this sentence is too specific, we can remove it, appending \textit{Let's think step by step} }after the prompt, does not lead to improvement.
% In order to explore the weakness reflected by the performance of ChatGPT on logical reasoning tasks, we conducted a thorough analysis over the generated responses under the two settings.

% As shown in Figure~\ref{fig:cot-example}\teng{the writing logic is not fluent here, why suddenly figure 1}, benefiting from instruction tuning~\citep{instructgpt}, ChatGPT is able to check the rationality of each option when given detailed prompting about step-by-step reasoning. 
% \teng{is this sent very important? It should be noted that the generated rationales are slightly different from the original definition~\citep{chain-of-thought}}. In arithmetic reasoning and commonsense reasoning, the chain of thoughts is often not mentioned in the context and question. Instead, the rationales are voluntarily generated via prompting and describe the possible reasoning path in an exploration space.
% In contrast, in logical reasoning of text, or more generally, in reading comprehension, all information is already given in the context and the reasoning process is inferring the relations among different pieces of facts mentioned in the passage.
% However, LLMs often fail to generate correction deductions based on the presented facts and rules in the context, leading to inaccurate prediction. 
% For example, on the right side of the example, though the final prediction is correct, the explanation of option B avoids discriminating the fallacy in the reasoning process.
% Indeed, option B is a plausible answer that it points out the unapproachability of paying low wages but fails to summarize the relation with reducing family's prosperity.
% Similar phenomenons are also observed in arithmetic reasoning and commonsense reasoning~\citep{self-consistency-wang2022}, where the final prediction seems correct but the intermediate reasoning process not.
% Motivated by this, we proposed to use zero-shot CoT as well as the self-consistency constraint~\citep{self-consistency-wang2022} to automatically generate reasonable explanations as prompts for few-shot CoT.
% We also proposed to incorporate the reasoning category information to help improve the generalization and quality of automatically generated CoT prompts.
% However, the experimental results show that using few-shot CoT prompting can only make marginal improvements over the vanilla few-shot baselines, where only the correct answer index is used in the prompt.
% In summary, we can draw two conclusions from the experiments: (1) LLMs often fail to make reasonable deductions based on observed facts and rules (zero-shot), and (2) LLMs struggle at capturing the logical reasoning process shown in the prompts and generalizing it to new problems. 

% Currently, trying to introduce logic prior via prompt engineering into LLMs can be quite difficult due to the API-based interaction manner, and LLMs' sensibility to different prompts and instructions.
% To this end, in this paper, we try to verify if the logic prior could be injected into LLMs while post-training.
% Specifically, we integrate MERIt~\citep{merit}, a self-supervised pre-training objective for logical reasoning, into FLAN-T5-3B~\citep{flan,flan-v2,t5}.
% % FLAN-T5-3B is an encoder-decoder LM with much fewer parameters. It is fine-tuned using billions of supervised datasets with synthetic instructions and can perform much better than larger models without supervised fine-tuning.
% % FLAN-T5-3B is an Encoder-Decoder LM with much fewer parameters but performs better than larger models that benefited from supervised instruction fine-tuning on various benchmarks.
% We test the performance of FLAB-T5-3B w/ MERIt on the logical reasoning benchmarks under both fine-tuning and in-context learning settings, respectively, and the results have demonstrated that logic-oriented self-supervised pre-training is still effective though built upon strong LLMs.
% In a nutshell, the contribution of this paper can be summarized as follows:
% \begin{enumerate}
%     \item We evaluated the capability of LLMs on logical reasoning benchmarks, demonstrating the significant gap between LLMs and previous SOTA approaches.
%     \item We have designed a series of experiments to reveal the weakness and instability of LLMs as well as CoT with respect to logical reasoning.
%     \item To bring more insights to the community, we try to introduce the data-driven approach into existing LLMs, and verified its effectiveness under both fine-tuning and in-context learning settings.
% \end{enumerate}




==> backs/1.intro.tex <==

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{image/intro_example_v1_0.pdf}
%     \caption{An instance of logical reasoning from the ReClor dataset. 
%     (i) represents the involved logical variable, e.g., entities or phrases. The reasoning structure is summarized at below.}
%     \label{fig:reclor-example}
%     \vspace{-0.3cm}
% \end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{image/zs-cot-example-v1-0.pdf}
    \caption{An example from ReClor dataset illustrating the prompting response under zero-shot and zero-shot CoT settings, respectively.}
    \label{fig:cot-example}
    \vspace{-0.3cm}
\end{figure*}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{image/Dingtalk_20230413185639.jpg}
%     \caption{An example of chain-of-thought prompting in arithmetic reasoning (math word problem solving.}
%     \label{fig:cot-math-example}
%     \vspace{-0.3cm}
% \end{figure}


\section{Introduction}
\label{sec:intro}
\input{tables/preliminary}

In the past few months, the released Large Language Models (LLMs), e.g., PaLM~\citep{palm}, \ding{LLAMA\citep{touvron2023llama}}, ChatGPT\footnote{https://openai.com/blog/chatgpt}, GPT-4\footnote{https://openai.com/product/gpt-4}, and Bard\footnote{https://bard.google.com/}, have surprised public greatly with fluently chatting, abundant world knowledge, strong ability of human assistance, as well as emergent complex capabilities such as arithmetic reasoning, commonsense reasoning, and logic.
However, considering the closed source of most of these largest models, systematic evaluation from different perspectives was once absent. Motivated by this, some recent studies have conducted series analysis over a wide range of NLP tasks~\citep{qin2023chatgpt-eval,bang2023chatgpt-eval,wang2023gcre-gpt,mt-chatgpt2023}, and the experimental results have revealed the gap between LLMs and previous state-of-the-art methods. 
Yet, for logical reasoning, most experiments focus on either simple discrete operations~\citep{qin2023chatgpt-eval} or those built on formal language~\citep{bang2023chatgpt-eval}, which is transformed from first-order logics via template based method.
% Yet, the logical ability of LLMs is still unexplored.  
Another category of logical reasoning problem is coupled with natural language, where the logical variables are often phrases, and can be difficult to be parsed into strict logic form. And it requires the understanding of natural language predicates, instead of logic operator.

In order to complete the evaluation of LLMs, we first conducted experiments on two natural language logical reasoning benchmarks, i.e., LogiQA-v2~\citep{logiqa} and ReClor~\citep{reclor} with zero-shot prompting and zero-shot Chain-of-Thought (CoT) prompting. 
As shown in Table~\ref{tab:pre-exp}, we can conclude that LLMs still perform much worse than the fine-tuned much smaller models on logical reasoning. 
Furthermore, utilizing zero-shot CoT, i.e., appending \textit{Let's think step by step} after the prompt, does not lead to improvement.
In order to explore the weakness reflected by the performance of ChatGPT on logical reasoning tasks, we conducted a thorough analysis over the generated responses under the two settings.

As shown in Figure~\ref{fig:cot-example}, benefiting from instruction tuning~\citep{instructgpt}, ChatGPT is able to check the rationality of each option when given detailed prompting about step-by-step reasoning. 
It should be noted that the generated rationales are slightly different from the original definition~\citep{chain-of-thought}. In arithmetic reasoning and commonsense reasoning, the chain of thoughts is often not mentioned in the context and question. Instead, the rationales are voluntarily generated via prompting and describe the possible reasoning path in an exploration space.
In contrast, in logical reasoning of text, or more generally, in reading comprehension, all information is already given in the context and the reasoning process is inferring the relations among different pieces of facts mentioned in the passage.
However, LLMs often fail to generate correction deductions based on the presented facts and rules in the context, leading to inaccurate prediction. 
For example, on the right side of the example, though the final prediction is correct, the explanation of option B avoids discriminating the fallacy in the reasoning process.
Indeed, option B is a plausible answer that it points out the unapproachability of paying low wages but fails to summarize the relation with reducing family's prosperity.
Similar phenomenons are also observed in arithmetic reasoning and commonsense reasoning~\citep{self-consistency-wang2022}, where the final prediction seems correct but the intermediate reasoning process not.
Motivated by this, we proposed to use zero-shot CoT as well as the self-consistency constraint~\citep{self-consistency-wang2022} to automatically generate reasonable explanations as prompts for few-shot CoT.
We also proposed to incorporate the reasoning category information to help improve the generalization and quality of automatically generated CoT prompts.
However, the experimental results show that using few-shot CoT prompting can only make marginal improvements over the vanilla few-shot baseline, where only the correct answer index is used in the prompt.
In summary, we can draw two conclusions from the experiments: (1) LLMs often fail to make reasonable deductions based on observed facts and rules (zero-shot), and (2) LLMs struggle at capturing the logical reasoning process shown in the prompts and generalize it new problems. 

Currently, trying to introduce logic prior via prompt engineering into LLMs can be quite difficult due to the API-based interaction manner, and LLMs' sensibility to different prompts and instructions.
To this end, in this paper, we try to verify if the logic prior could be injected into LLMs while post-training.
Specifically, we integrate MERIt~\citep{merit}, a self-supervised pre-training objective for logical reasoning, into FLAN-T5-3B~\citep{flan,flan-v2,t5}.
% FLAN-T5-3B is an encoder-decoder LM with much fewer parameters. It is fine-tuned using billions of supervised datasets with synthetic instructions and can perform much better than larger models without supervised fine-tuning.
% FLAN-T5-3B is an Encoder-Decoder LM with much fewer parameters but performs better than larger models that benefited from supervised instruction fine-tuning on various benchmarks.
We test the performance of FLAB-T5-3B w/ MERIt on the logical reasoning benchmarks under both fine-tuning and in-context learning settings, respectively, and the results have demonstrated that logic-oriented self-supervised pre-training is still effective though built upon strong LLMs.
In a nutshell, the contribution of this paper can be summarized as follows:
\begin{enumerate}
    \item We evaluated the capability of LLMs on logical reasoning benchmarks, demonstrating the significant gap between LLMs and previous SOTA approaches.
    \item We have designed a series of experiments to reveal the weakness and instability of LLMs as well as CoT with respect to logical reasoning.
    \item To bring more insights to the community, we try to introduce the data-driven approach into existing LLMs, and verified its effectiveness under both fine-tuning and in-context learning settings.
\end{enumerate}







==> backs/abstract-v1.tex <==
\begin{abstract}
% Recent research progress over natural language processing demonstrates a huge impact due to the emergent capability of Large Language Models (LLMs). LLMs can perform very well on various tasks using only few labeled samples as prompts without task-specific fine-tuning. 
% Specifically, with the help of Chain-of-Thought (CoT), previous study show that LLMs are also able to conduct multi-step arithmetic reasoning and commonsense reasoning. 
% However, in our preliminary experiments on the logical reasoning tasks, we find that LLMs cannot outperform the much smaller language models with fine-tuning, e.g., RoBERTa-Large.
% Furthermore, even CoT does not make significant improvements. 
% To this end, in this paper, we aim to explore the possible reasons why LLMs perform much worse on logical reasoning of text.
% Besides, considering the constraints brought by API-based usage and LLMs' sensitivity to prompts and instructions, we also try to provide some insights to future research by exploring if any of previous data-driven approaches can still benefit LLMs with logical reasoning capability. 
% Specifically, we present LogicLLM by combining logic-reasoning-oriented self-supervised pre-training with off-the-shelf LLMs. 


Existing efforts to improve logical reasoning ability of language models have predominantly relied on supervised fine-tuning, hindering generalization to new domains and/or tasks. The development of Large Language Models (LLMs) has demonstrated the capacity of compressing abundant knowledge into a single proxy, enabling them to tackle multiple tasks effectively. 
% However, our preliminary experiments reveal the weakness of LLMs on logical reasoning. 
Our preliminary experiments, nevertheless, show that 
the performance of LLMs on logical reasoning benchmarks is far behind the existing state-of-the-art baselines.
%LLMs do not present strong capability on logical reasoning.
% In this paper, we make the first attempt to investigate the feasibility of incorporating logical knowledge through self-supervised post-training, and activating it via in-context learning, which we termed as LogicLLM.


In this paper, we make the first attempt to investigate the feasibility of building a fully self-supervised framework for incorporating logical reasoning capability into LLMs, and activating it via in-context learning, which we termed as LogicLLM.
Specifically, we devise an auto-regressive objective variant of MERIt~\citep{merit} and integrate it with two LLM series, i.e., FLAN-T5 and LLaMA, with parameter size ranging from 3 billion to 30 billion.
The results on multiple challenging logical reasoning benchmarks demonstrate the effectiveness of LogicLLM.
%\jiao{[I think now we could highlight our results here.]
% Particularly, our LogicLLMs based on \flant-11B achieved comparable performance with ChatGPT on ReClor and LogiQA-v2. 
% % And the one based on \llama-30B can outperform \llama-65B as well as Falcon-40B, verifying the feasibility of building fully self-supervised meta-training framework to enhance LLMs with particular capabilities.
% And the performance on MMLU and Big-Bench-Hard has verified the framework does no damage to the general capabilities.
Specifically, our LogicLLMs, which are built upon \flant-11B, have achieved performance comparable to ChatGPT on ReClor and LogiQA-v2. Additionally, the results of \llama-based models obtained from MMLU and Big-Bench-Hard confirm that the framework does not compromise the model's overall capabilities.
%}
Besides, we conduct extensive ablation studies to analyze the key factors in designing logic-oriented proxy tasks. 
% We also discussed the limitations of current training method to provide some insights to future research.
\footnote{The code, training data, and trained models will be released upon publication.%at~\href{https://github.com/SparkJiao/MERIt-v2}{github.com/SparkJiao/MERIt-v2.}
}
% Particularly, our LogicLLM outperforms ChatGPT's zero-shot logic reasoning  performances on  the two investigated benchmarks. 
\end{abstract}

==> backs/aug.tex <==
\iffalse
Though the implementation of auto-regressive generative training is simple, it can be more possible to be mislead to memorization instead of logical reasoning.
Taking a corner case as example, when the logically consistent instance pair has covered all the sentences in the paragraph, the self-supervised task is then degraded into simple paragraph completion by recovering the compressed knowledge from the pre-training stage.
\fi 

==> backs/exp.tex <==
\input{tables/main_res}
\input{tables/llama_main}


\section{Experiment}

\subsection{Foundation Model and Evaluation Benchmark}

We incorporate our pre-training approach into two representative LLMs, namely, LLaMA~\citep{touvron2023llama} and FLAN-T5~\citep{flan}. These models have parameters ranging from 3 billion to 13 billion.
To test the logical reasoning capabilities from different perspectives, we have selected four datasets spanning three categories. ReClor~\citep{reclor} and Logiqa-V2~\citep{logiqa} are two logical reasoning benchmarks, sourced respectively from standardized graduate admission examinations and logical examination papers intended for reading comprehension. 
DREAM~\citep{dream} is a dataset focusing on hybrid reasoning benchmarks, and we use it to evaluate if our proposed approach can also benefit general natural language reasoning. BIG-Bench-Hard is a series of challenging tasks for LLMs \citep{big-bench-hard}. We employ this dataset to test whether the model can apply logical reasoning to complex tasks, such as causal judgment and tracking shuffled objects, and to explore which tasks or abilities might be negatively impacted by logic-oriented pre-training.

% \subsection{Data and Baseline}

% We evaluated the LLMs and FLAN-T5-3B on two logical reasoning benchmarks, ReClor~\citep{reclor} and LogiQA-v2\footnote{https://github.com/csitfun/LogiQA2.0/}. The former is extracted from the logical reasoning question of standardized graduate admission examinations, while the latter one is sourced from publicly available logical examination papers for reading comprehension, which is designed by domain experts for evaluating the logical reasoning ability and test participants. The examinations are in Chinese and translated into English by experts.

% For the baselines, we mainly test the performance of ChatGPT, which is referred as GPT-3.5-turbo. Our ablation studies are conducted taking FLAN-t5-3B~\citep{flan} as the foundation model.

\subsection{Implementation Details}
\teng{We should talk about the data,  the training settings and the evaluation metrics. }
% For the hyperparameters of the ChatGPT API service, we set the number of maximum generated tokens as 2048 and the temperature of decoding is set to 0.0. 

\noindent \textbf{Data} We use the FLAN collection and MERIT corpus to perform logic-oriented pre-training. The FLAN Collection

During the post-training of FLAN-T5-3B, the batch size is set to 4096. We use gradient accumulation to enlarge it while the actual batch size on each device is set to 1. The maximum length for sequences from the FLAN corpus and MERIt corpus is set to 1024 and 512, respectively. We used a learning rate of 1e-4 and the training process lasted 32 hours on 8 NVIDIA A100 80G GPUs. For FLAN-T5 series, we find that pre-training on non-instructed data will hurt the instruction following ability of models. To this end, we randomly sample a subset of FLAN collection following the pre-defined task data ratios and train the model in multi-task setting. Since FLAN collection is mainly composed of supervised data, we add the baseline continued trained with FLAN data to discuss the possible influence.

For each dataset, we use exactly the same instructions and few-shot samples accross different models to make fair comparison. During the test of BIG-Bench-hard, we used the officially provided annotated exemplars for both (direct) few-shot and CoT evaluation.

% During fine-tuning on the ReClor dataset, the learning rate is set to 3e-5 and the batch size is set to 8. The models are fine-tuned with 10 epochs.


\section{Results and Analysis}
% \input{tables/cot}
\input{tables/flan-t5-bbh}


\subsection{Overall Results}

\subsubsection{Logical Reasoning}

As shown in Table~\ref{tab:mcqa}, on ReClor and LogiQA-v2, FLAN-T5 w/ MERIt can achieve better performance compared with both FLAN-T5 and FLAN-T5 + FLAN on most dataset splits. LLaMA w/ MERIt also achieved certain improvements but the absolute accuracy is limited, which is consistent with the observations in emergent abilities~\citep{emergent2022jason}. Overall, from the results we can conclude that 
(1) instruction-tuning on multiple supervised datasets, i.e., FLAN collection, is still insufficient for learning logic. Since FLAN has included some reasoning data, the reason can be the sparsity of reasoning relevant data in the whole collection, and the conflicts between different tasks. 
(2) With logic-enhanced training, FLAN-T5-11B w/ MERIt + FLAN can obtain comparable performance under zero-shot setting with ChatGPT. 
(3) We have also tested the performance under 3-shot setting on FLAN-T5-3B. Though improvements are also observed compared with the ones without MERIt, the accuracy is similar to that under zero-shot setting, demonstrating that how to select and generalize from the exemplars are still an open problem to be solved. We leave this as the future work. 
% (4) 

\subsubsection{General Reasoning and Application}

Beside logical reasoning of text, we also care about if the learned logical reasoning capability could be applied in general reasoning process. To this end, we evaluate the enhanced LLMs on DREAM, a dialogue based reasoning dataset. For FLAN-T5 series, we find that the grades are nearly saturated, possibly because FLAN-collection has already included many reading comprehension and reasoning datasets. As a result, the improvements brought by MERIt are marginal.
However, on LLaMA series, the improvements are really significant. And the margin also increases when scaled the parameters are scaled from 7 billion to 13 billion, demonstrating the effectiveness and generalization of logic-enhanced training for LLMs.

Besides, we also evaluated the performance of trained models on BIG-Bench-Hard, 


% \subsection{Ablation Studies}

% \subsection{Influence of Auxiliary Instruction Tuning}

% Take the results about FLAN-T5 + MERIt and LLaMA + GPT4ALL + MERIt

\input{tables/cot}



\subsection{Weakness of LLMs on Logical Reasoning}

As displayed in Table~\ref{tab:cot}, we also evaluated the performance of LLMs under few-shot and CoT setting. 
The intermediate reasoning process is automatically generated by ChatGPT via prompting through \textit{Let's think step by step}. For zero-shot CoT, we directly append an suffix prompt - \textit{So the answer is} to guide the models to summarize and conclude the answer. For few-shot CoT, the reasoning process is first generated for each sample in the training set. Then we keep the samples where the final prediction is correct following the steps in zero-shot CoT.
Finally, during test, we randomly select the samples from the kept candidates as well as the automatically generated CoT as exemplars.
However, we find that both few-shot and using CoT cannot significantly benefit the models. One possible reason is the selected samples are far dissimilar to the target example. To verify it, we include the reasoning category information during exemplar selection. In Logiqa-V2, each question is also annotated with the reasoning category, e.g., categorical reasoning, sufficient conditional reasoning, and necessary conditional reasoning. During exemplar selection, only those sharing at least two common reasoning categories will serve as the candidates for few-shot CoT prompting. The method variant is denoted as ChatGPT w/ CoT + Cate. in the table. 
Nevertheless, we find that carefully selecting prompting exemplars also provides limited bonus. All the results suggest that LLMs fail to parse the reasoning structure from limited observed examples. As a result, they cannot learn both the input-label and input-rationale-label mapping inline. And we can observe from Table~\ref{tab:mcqa} that MERIt also contribute a little to this problem. We leave this to future work.




% \subsection{Human Evaluation of Generated CoT}

% \subsection{Effect of Improved CoT}

% Table~\ref{tab:cot} shows the results of ChatGPT under both zero-shot and few-shot settings.
% % GPT-3.5-turbo w/L-CoT refers to logically enhanced CoT, i.e., automatic CoT augmented self-consistency constraints. 
% It can be observed that few-shot CoT achieves better results on both benchmarks, demonstrating the effectiveness of improved rationales. The phenomenon also indicates that LLMs often fails to generate correct deductions with the given facts and rules. However, the improvements over the vanilla few-shot baseline are quiet marginal, which reveals that language modeling can hardly distil the reasoning structure from observed examples and generalize it to new examples.

% Another concern is that randomly sampled examples for prompt may lead to bias because reasoning is often complex, and different problems would rely on different reasoning tecniques. To solve this problem, we utilize the reasoning category annotations in LogiQA-v2. Each sample in LogiQA-v2 has been annotated with the specific reasoning category, e.g., categorical reasoning, sufficient conditional reasoning, and necessary conditional reasoning. Then we can select the examples sharing at least 2 common reasoning categories with the anchor example as the prompt to alleviate the bias. The method is annotated as w/ CoT + Cate.. Nevertheless, the results are still comparable to w/ CoT and vanilla few-shot baseline, which also verify the above the conclusion that purely language modeling cannot help models expose the internal reasoning structure.

% \subsection{Analysis of Logical Reasoning Oriented Pre-training}

% The results of models combined with MERIt are shown in Table~\ref{tab:mcqa}. From the table we can conclude that: (1) though the data-driven approach use only self-supervised training data from a general domain (Wikipedia), it can still benefit the strong language model. The results also indicate that current language models still lack necessary prior knowledge about logical reasoning. 
% % (2) The improvement of CoT is limited. As displayed in Figure~\ref{fig:cot-example}, this may imply that LLMs are not good at combining existing information to deduce new conclusions. The deduced plausible thoughts in turn lead to unexpected noise in the language modeling process. 
% (2) Post-training using the MERIt corpus with the auto-regressive objective can also improve performance under in-context learning. This is possible because the counterfactual data augmentation strategy can promote the relation-centric reasoning process and the recognition of logical variables in natural language. 
% (3) The original contrastive learning objective does not make significant improvements to the overall results. We attribute this to its gap with the auto-regressive decoding strategy.


% \ding{Analysis needs to be in-depth. It's better to have some data visualization. Demonstrate what have been improved. And analyze from a theoretical perspective like inductive reasoning and deductive reasoning. }

% \ding{need to have a good conclusion. What's the impact of this work? Pave the way for xxxx / shed the light on xxxx}

==> backs/intro-0615.tex <==

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{image/intro_example_v1_0.pdf}
%     \caption{An instance of logical reasoning from the ReClor dataset. 
%     (i) represents the involved logical variable, e.g., entities or phrases. The reasoning structure is summarized at below.}
%     \label{fig:reclor-example}
%     \vspace{-0.3cm}
% \end{figure}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{image/zs-cot-example-v1-0.pdf}
%     \caption{An example from ReClor dataset illustrating the prompting response under zero-shot and zero-shot CoT settings, respectively.}
%     \label{fig:cot-example}
%     \vspace{-0.3cm}
% \end{figure*}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{image/Dingtalk_20230413185639.jpg}
%     \caption{An example of chain-of-thought prompting in arithmetic reasoning (math word problem solving.}
%     \label{fig:cot-math-example}
%     \vspace{-0.3cm}
% \end{figure}


\section{Introduction}
\label{sec:intro}
% \input{tables/preliminary}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/preliminary_image_v1_4.png}
    \caption{The overall accuracy of LLMs, i.e., ChatGPT (GPT-3.5-turbo) and LLaMA, and existing state-of-the-art methods~\cite{merit} on logical reasoning benchmarks. Specifically, for \llama, we evaluate the performance of models with different parameter size, i.e., 7B, 13B and 33B. The evaluation of LLMs follows zero-shot in-context learning setting, where the models are expected to decode the answer based on the given instruction, context, and question.}
    \label{fig:pre-exp}
    \vspace{-0.5cm}
\end{figure}

% \ding{missing citations for some papers like Lets think step by step}\\
% \ding{no figures or data visualization. Very content heavy and very dry for reviewers. Need to work on the presentation after the arxiv deadline}\\
% \ding{Not enough insights. Should think about how to make the analysis more attractive and interesting after arxiv deadline}\\
% \ding{The second question is not very clear. can the
% introduced logic knowledge be generalized to hy-
% brid tasks? What does hybrid task mean? Refine after arxiv deadline}


% \ding{The whole Intro needs to rewrite. It sounds like an evaluation only. Need to have a good story to convince the reviewers. The paper title is also too plain. You need a good title to attract attention.}

% \ding{A proposed storyline for the paper: 1. Talk about the progress of logical reasoning in NLP. Why logical reasoning is important and what were the methods? 2. LLMs have pushed the performance of  reasoning, can include numerical reasoning, xxx reasoning. You can mention related works like PAL, etc. Talk about how they differentiate with the traditional methods. 3. However, there is a lack of systematic evaluation of logical reasoning / LLMs are still weak in logical reasoning. 4. What is missing / What is the gap to be closed? Why is it important to do so? 5. Mention what you have done and your insights and contribution briefly.}


% \ding{Here are a few possible paraphrased versions of the paper title to make it more attention-grabbing:$
% "Why Logic-enhanced Training is a Game-Changer for Large Language Models"
% "Revolutionizing Language Models: The Crucial Role of Logic-enhanced Training"
% "Unleashing the Full Potential of Language Models with Logic-enhanced Training"
% "Logic + Language: The Winning Combination for Next-gen AI Training"
% "Breaking Barriers: How Logic-enhanced Training Takes Language Models to New Heights"
% "Why Logic-enhanced Training is Critical for Empowering Large Language Models"
% "Unleashing the Full Potential of Language Models with Logic-enhanced Training"
% "Revolutionizing Language Learning: The Importance of Logic-enhanced Training for Large Language Models"
% "Going Beyond Traditional Methods: How Logic-enhanced Training Improves Large Language Models"
% "The Logic Revolution: Why Large Language Models Need Logic-enhanced Training to Succeed"
% "Mastering Language: Enhancing Large Language Models with Logic-based Training"
% "Logic Meets Language: The Game-changing Approach to Training Large Language Models"
% "From Good to Great: How Logic-enhanced Training Takes Large Language Models to the Next Level"
% "Transforming Language Understanding with Logic-enhanced Training for Large Language Models"
% "Breaking the Limits: The Necessity of Logic-enhanced Training for Large Language Models".$}


% Version v2.0
Logical reasoning has long been treated as a complex yet essential  ability in cognition that goes beyond fundamental language understanding. It also serves as a necessary foundation in negotiation, debate and writing~\citep{reclor}. Thus, 
extensive efforts have been made in recent years to enhance logical reasoning ability of language models. 
% \joty{The following sentence came quite abruptly. You could start like this..Earlier approaches fine-tune a pretrained LM. ....\cite{}. However, this requires ...} 
Previous approaches have primarily focused on incorporating the knowledge about logic. For instance, some have utilized graph neural networks to acquire relational representations of semantic elements~\citep{dagn-huang-2021}, while others have employed data augmentation techniques to introduce first-order logic~\citep{lreasoner}. 
However, these approaches still require a substantial amount of annotated training data for fine-tuning, which restricts the model's ability to generalize to new tasks due to discrepancies in data distribution and optimization objectives.
% However, fine-tuning based approach requires reasonable amount of annotated training data, and hinders the model to generalize to new tasks due to the mismatch of data distribution and optimization objective.
% , e.g., fine-tuning on multiple choice question answering and predicting on natural language inference task. 

On the other hand, the recent development of Large Language Models (LLMs), e.g., PaLM~\citep{palm}, LLAMA\citep{touvron2023llama}, ChatGPT\footnote{https://openai.com/blog/chatgpt}, GPT-4 \cite{openai2023gpt}\footnote{https://openai.com/product/gpt-4}, and Bard\footnote{https://bard.google.com/}, suggests that LLMs can serve as a proxy to compress abundant knowledge, and solve various tasks following human instructions with less  specialization. However, as shown in Table \ref{fig:pre-exp}, our  experiments on logical reasoning benchmarks reveal that LLMs also lack the ability to do logical reasoning. There are also results showing that the promotion brought by few-shot exemplars or Chain-of-Thought (CoT) prompting \citep{chain-of-thought} is also limited~\citep{agi-eval2023zhong}.
% \joty{You need to cite those evidences.}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{image/logiqa-sample-v2.pdf}
    \caption{An example logical reasoning from LogiQA-v2 dataset \citep{logiqa}. The relations between different constituents, e.g., \textit{agriculture} and \textit{development of Andean society}, include various predicates, and the example can be hard to converted into logical form through either first-order logic or formal language.
    % The question can be hard to be expressed in symbolic language due to multiple different predicates and phrases. \joty{double check the example? Do you mean the question is hard? or something else?}
    }
    \label{fig:logiqa-sample}
    \vspace{-0.5cm}
\end{figure}
% As demonstrated by the evaluations on various benchmarks~\citep{qin2023chatgpt-eval,bang2023chatgpt-eval,wang2023gcre-gpt,mt-chatgpt2023}, logic is not the only knowledge that LLMs are short of, e.g., arithmetic reasoning and knowledge grounding.
% In order to mitigate the absence of specific complex capability and avoid using too much annotated data, some work tends to employ external tools, or calling predefined API, such as search engine (information retriever)~\citep{toolformer,arm-survey-lecun}, SQL query~\citep{binder2022cheng}, or calculator~\citep{pal2022gao,pot2022chen}. 
% The advantage is that the external tools or APIs can provide accurate results with explicable execution steps, and decouple the complex inference process with semantic understanding and parsing, which the LLMs are more capable on.
% % Though promising, similar methodology can be circumscribed when applied to logical reasoning. The tool-based hybrid system requires both finite operation space and execution steps, e.g., the scenarios where the premises are translated from first-order logic or symbolic systems. 
% Though promising, similar methodology can be circumscribed when applied to logical reasoning of text. The tool-based hybrid system requires both well-defined executor and explicit arguments. For example, it can be more suitable for the first-order logic presented with formal language and symbols.
% However, in natural language based logical reasoning, the logical variables could be arbitrary entities and phrases, leading to extreme difficulty in building executable symbolic logical reasoners. 
% % \teng{this paragraph can be kept}

% Rewrite here 0521
As the example shown in Figure~\ref{fig:logiqa-sample}, logical reasoning in natural language can be challenging due to the various relations and expressions involved, which are difficult to transcribe into symbolic or formal languages. Existing work that aims to enhance particular capabilities of LLMs can be categorized into two broad approaches. The first category relies on external tools or APIs, such as search engine (information retriever)~\citep{toolformer,arm-survey-lecun}, SQL query~\citep{binder2022cheng}, or calculator~\citep{pal2022gao,pot2022chen}. These approaches allow LLMs to focus on argument parsing and semantic understanding, resulting in more accurate step-by-step results compared to those generated through auto-regressive decoding. 
However, it can be circumscribed when applied to logical reasoning due to the absence of explicit symbolic or formal language for problem description.
Another approach is instruction tuning, involving augmenting data from existing datasets~\citep{aribandi2022ext5,flan,flan-v2,zeroprompt,sanh2022multitask-t0} or annotating human queries with high quality responses and/or human feedback~\citep{self-instruct2022wang,wizardlm2023xu}, which is also non-trivial for logical reasoning given its sparsity and high annotation cost.
% Collecting relevant instruction tuning data for logical reasoning is challenging due to . Therefore, enhancing the logical reasoning ability of LLMs through a data-driven approach remains non-trivial.

% To this end, in this paper, we aim to explore if the logic-enhanced training could help introduce logic prior into LLMs and keep the generalization as much as possible. 
% To this end, in this paper, we aim to explore logic-enhanced training for LLMs and keep the generalization as much as possible.
% In this paper, we aim to explore the logic-enhanced training for LLMs.
% Nevertheless, most methods focusing on data augmentation or synthesis~\citep{lreasoner} have significant mismatch on training objectives with causal language modeling, \jiao{I need two motivations here.}, and may cause the degradation of in-context learning.
% To tackle the above problems, we proposed a auto-regressive version of MERIt~\citep{merit}, a self-supervised pre-training method for logical reasoning, which is originally designed as contrastive learning.
% Recent work activating the potential ability of LLMs mostly rely on supervised instruction tuning\footnote{In this paper, we use \textit{supervised fine-tuning} to refer the training process rely on labels annotated by human and LLMs. \textit{Self-supervised} training is also supervised learning but the labels are constructed from natural data.}~\citep{instructgpt}. Through either template-based task-specific data~\citep{aribandi2022ext5,flan,flan-v2,zeroprompt,sanh2022multitask-t0} or open-domain instruction-response pairs~\citep{self-instruct2022wang,wizardlm2023xu}, they all rely on high quality annotations from human expert or teacher LLMs, leading to high difficulty and cost in collecting logic-specific data.
% In order to alleviate the data sparsity, we propose to post-train LLMs via self-supervised objectives. Specifically, we introduce MERIt~\cite{merit}, a self-supervised pre-training method for logical reasoning, which was originally designed as contrastive learning. We have explored both the original framework and the auto-regressive variant to seek the trade-off between computation overhead and the benefits.
% % \teng{Besides, the data for MERIt training is constructed from Wikipedia, which can help avoid the over-fitting to specific domain: do not need?}. 
% We test the performance based on FLAN-T5~\citep{flan-v2} and LLaMA~\citep{touvron2023llama}, with model sizes ranging from 3 billion to 13 billion to verify its scabalility.
% In this paper, we aim to explore the logic-enhanced meta-training\footnote{https://github.com/allenai/acl2022-zerofewshot-tutorial.} \joty{this is better called as `meta-training'? (do not confuse with meta learning)}\jiao{I'm not sure. I need find some papers to cite. Maybe I citation information next time.} for LLMs.
In this paper, we aim to explore the \textbf{self-supervised} logic-enhanced meta-training\footnote{https://github.com/allenai/acl2022-zerofewshot-tutorial.} for LLMs.
% , where the LLMs are first trained through self-supervised learning and directly evaluated on logical reasoning benchmarks.
As exemplified above, processing the diverse relational expressions entailed in natural language in a key challenge to enhance logical reasoning. To address this, we introduce \meritp, a self-supervised pre-training method by relation discrimination. 
% \joty{It's better to say \merit+.} The \joty{original \merit~\citep{merit}}  
The original \merit~framework includes data construction for contrastive learning and counterfactual data augmentation for eliminating information shortcut. The positive instance is a set of sentences describing the relation between an anchor entity pair from two different views, where one view is direct and the other is indirect. And the negative instances are synthesized via relation editing. The counterfactual data augmentation further emphasizes the relation-centric reasoning process with entity replacement to remove the bias from world knowledge.
% \joty{I rewrote it as follows}. 
However, the contrastive learning objective could be inconsistent with auto-regressive decoding, and the computation complexity grows exponentially with the number of negative candidates.   
%And negative candidates bring exponential increase in computation. 
% As a result, we propose an auto-regressive variant by directly optmizing on the positive instance.
In \merit+, we propose an auto-regressive variant by directly optimizing on the positive instance. Specifically, given a direct/indirect description about the anchor entity pair, the model is asked to generate the indirect/direct one via auto-regressive decoding. The entity replacement-based counterfactual data augmentation is kept to make sure LLM cannot copy the results from its memory.
% We have explored both the original framework and the auto-regressive variant to seek the trade-off between computation overhead and the benefits.
The experiments are conducted on two LLM series, FLAN-T5~\citep{flan-v2} and LLaMA~\citep{touvron2023llama}, with different parameter sizes.

% The experimental results on two logical reasoning benchmark demonstrates the effectiveness of our proposed method.
% and verified the feasibility and necessity of logic-enhanced training for LLMs. 
% Besides, the improvements under in-context learning also suggest the feasibility to augment complex ability of LLMs without supervised fine-tuning.
% Finally, we have discussed the possible factors relevant to logic prior in raw text corpus and the weakness of current LLMs on logical reasoning.
We design experiments to study two questions: (1) is it feasible to enhance logic ability via only self-supervised meta-training for LLMs, i.e., without task-specific supervised fine-tuning? and (2) does the logic-enhanced training improves the general language understanding of LLMs?
For the first question, we find that the LLMs with the \meritp~objective performs better on logical reasoning benchmarks without the need of further fine-tuning. 
% Particular, LLaMA-based models achieves better accuracy without open-domain instruction tuning.
As for the second question, we find that the learned logic ability also boosts the performance on general language understanding. i.e., MMLU~\citep{mmlu2021} and BIG-Bench-Hard~\citep{big-bench-hard}.
The contributions of this paper can be summarized as follows:
\begin{enumerate}
    \item We evaluate the capability of LLMs on logical reasoning benchmarks, demonstrating weakness of LLMs on logical reasoning.
    \item We propose an auto-regressive and self-supervised framework for logic-enhanced meta-training, \merit+, and our experiments have verified the feasibility to introduce complex ability into LLMs without task-specific fine-tuning.
    % \item To bring more insights to the community, we try to introduce the data-driven approach into existing LLMs, and verified its effectiveness under both fine-tuning and in-context learning settings.
    \item We conduct extensive experiments on both FLAN-T5 and LLaMA series, with model parameter sizes ranging from 3 to 30 billion. The results on logical reasoning and massive language understanding demonstrate the effectiveness of our approach. We have also explored the possible effects of different pre-training strategies to bring in some insights to future research.
\end{enumerate}
% \teng{still need more polishing, i will do another round probably on 11-May-2023.}




==> backs/intro-0620.tex <==
\section{Introduction}
\label{sec:intro}
% \input{tables/preliminary}
\input{figures/logicqa-example}
Logical reasoning, a complex but essential cognitive ability extending beyond basic language understanding, serves as a critical foundation for negotiation, debate, and writing~\citep{reclor}. Figure~\ref{fig:logiqa-sample} shows an example of logic reasoning in natural language. This tasks presents challenges due to diverse relations and expressions, which are difficult to convert into symbolic or formal languages. 
 Consequently, numerous efforts have been made to bolster logical reasoning in language models. 
% \joty{The following sentence came quite abruptly. You could start like this..Earlier approaches fine-tune a pretrained LM. ....\cite{}. However, this requires ...} 
Traditionally, these efforts have aimed to incorporate logic knowledge. For example, ~\citet{dagn-huang-2021} employed graph neural networks to capture relational representations of semantic elements, while ~\citet{lreasoner} leveraged data augmentation techniques to integrate first-order logic. However, these methods necessitate significant amounts of annotated training data for fine-tuning. This requirement restricts the model's ability to generalize to new tasks, due to discrepancies in data distribution and optimization objectives.

Conversely, recent advancements in Large Language Models (LLMs), such as PaLM~\citep{palm}, LLaMA~\citep{touvron2023llama}, ChatGPT\footnote{https://openai.com/blog/chatgpt}, GPT-4 ~\cite{openai2023gpt}, and Bard\footnote{https://bard.google.com/}, suggest an alternative approach. These LLMs function as proxies that encapsulate vast amounts of knowledge and tackle various tasks with minimal specialization, guided by human instructions. Despite their promise, our preliminary experiments on logical reasoning benchmarks 
% depicted in Figure~\ref{fig:pre-exp}, 
expose a deficiency in LLMs' logical reasoning capabilities.
% \teng{Can be more specific by citing the numbers in Figure 2}. 
Specifically, \llama-7B falls behind the simple RoBERTa-Large~\citep{roberta} with more than 20 points on LogiQA-v2 and ReClor, while the latter model has only 360M parameters as shown in Table \ref{tab:pre-exp} in the appendix. %And even ChatGPT leaves a margin with 6.6 points with the supervised finetuing SOTA model based on RoBERTa-Large on LogiQA-v2.
Further, the limited improvements achieved through few-shot exemplars or Chain-of-Thought (CoT) prompting~\citep{chain-of-thought} echo these findings~\citep{agi-eval2023zhong}. 
% \joty{You need to cite those evidences.}

% \input{figures/pre-exp}
% \teng{Can move the next paragraph to the related work section?} 
Current to bolster specific capabilities of LLMs generally fall into two categories. The first approach uses external tools or APIs~\citep{toolformer,arm-survey-lecun,binder2022cheng,pal2022gao,pot2022chen}. These tools assist LLMs in argument parsing and semantic understanding, improving step-by-step results. However, their usefulness for logical reasoning is constrained by the absence of a symbolic language for problem descriptions. The second approach, instruction tuning, employs data augmentation or enriched human feedback. But it faces challenges due to the scarcity of relevant data and high annotation costs~\citep{instructgpt,wizardlm2023xu}. 
% \teng{add references for the second approach?}

\teng{Rewrite the whole paragraph. Todo later!}
In this paper, we concentrate on exploring self-supervised logic-enhanced meta-training for LLMs. A primary challenge lies in handling the variety of relational expressions intrinsic to natural language, which are vital for improving logical reasoning. Recognizing this importance, we present \meritp, a novel self-supervised pre-training approach based on logic-consistent relation learning. This innovative method enhances the logical reasoning abilities of LLMs, facilitating their understanding of various relational nuances in data, and thereby improving their semantic comprehension and inference-making capabilities. 
% \meritp~ is independent of specific logic reasoning tasks and does not require supervised annotations,  therefore making it easy to generalize to new logic reasoning tasks. 
Our approach is designed to be task-agnostic, and it eliminates the need for annotations, making it highly adaptable to new logic reasoning tasks.
% \joty{It's better to say \merit+.} The \joty{original \merit~\citep{merit}}  
% The original \merit~framework~\citep{merit} combines the process of data construction for contrastive learning along with counterfactual data augmentation to prevent information shortcut. In this context, the positive instance comprises sentences that describe the relationship between an anchor entity pair from two distinct perspectives - direct and indirect. In contrast, the negative instances are synthesized through the process of relation editing. %By emphasizing the difference in these relations, we facilitate the model's capacity for logical reasoning.
Specifically, we search positive instance pair from Wikipedia documents that comprises sentences describing the relationship between an anchor entity pair from two distinct perspectives - direct and indirect.
Additionally, to underscore the relation-centric reasoning process and to prevent memorization problem, we utilize entity replacement within the counterfactual data augmentation method. 
While enhancing the logical comprehension of the model, this approach also confronts issues of potential bias and inference shortcuts. 
% \joty{I rewrote it as follows}. 
% Despite these advancements, the contrastive learning objective is inconsistent with auto-regressive decoding, and the computational complexity increases   with the growing number of negative candidates.  %\teng{why exponentially? do we have experiments to support this claim? \jiao{I think this is intuitive giving $O(N^2)$ memory/time complexity with the sequence length $N$.}}
The original \merit~framework employs contrastive learning to keep consistent with downstream task format, which, however, can hurt the in-context learning ability, and introduce extra computation overhead.
\merit+ address these challenges by using an auto-regressive objective that optimizes directly on the positive instance. Specifically, given a direct or indirect description about the anchor entity pair, the model is tasked to generate the other perspective (indirect or direct) via auto-regressive decoding. The entity replacement-based counterfactual data augmentation is retained to prevent the LLM from merely reproducing results from its memory, thereby preserving the logic-enhanced aspect of the learning process. Additionally, \meritp~waives the relation annotation from external knowledge base, ensuring fully self-supervised process.

We conducted experiments across two distinct LLM series, FLAN-T5~\citep{flan-v2} and LLaMA~\citep{touvron2023llama}, encompassing a variety of parameter sizes. These experiments were designed to investigate two main questions: (1) Can the logical reasoning capabilities be exclusively improved through self-supervised meta-training for LLMs, thereby circumventing the need for task-specific supervised fine-tuning? (2) Does incorporating logic-enhanced training improve the overall language understanding capabilities of LLMs?

In response to the first question, our findings suggest that LLMs trained with the \meritp~objective demonstrate superior performance on logical reasoning benchmarks, eliminating the need for further fine-tuning. Our LogicLLMs based on \flant-11B attain comparable results to ChatGPT on two logic reasoning benchmarks, ReClor~\citep{reclor} and LogiQA-v2~\citep{logiqa2}, highlighting the feasibility of enhancing logical reasoning abilities through self-supervised training alone.

Regarding the second question, our evaluations with \llama-based models on three general language understanding benchmarks - RACE~\cite{race}, MMLU~\citep{mmlu2021} and BIG-Bench-Hard~\citep{big-bench-hard}, confirm that the enhanced logical reasoning capabilities don't compromise the model's overall language understanding on MMLU and BBH. In fact, the learned logic ability appears to boost the model's performance in RACE.
%\teng{Remove the contribution part?}
\iffalse
The contributions of this paper can be summarized as follows:

\begin{itemize} 
\itemsep0em 
\item We examine the proficiency of LLMs on logical reasoning benchmarks, thereby identifying the current shortcomings of LLMs in terms of logical reasoning.
\item We introduce \merit+, an auto-regressive and self-supervised framework for logic-enhanced meta-training. Our experiments validate the feasibility of instilling complex logical reasoning abilities into LLMs without the need for task-specific fine-tuning.
\item We carry out comprehensive experiments on both FLAN-T5 and LLaMA series, with model parameter sizes ranging from 3 to 33 billion. The results from both logical reasoning and massive language understanding tasks affirm the effectiveness of our proposed approach. Additionally, we investigate the potential effects of various pre-training strategies, providing valuable insights for future research.
\end{itemize}
\fi 
%\teng{Done! The current version is too long, need to reduce half page}




==> backs/method-0615.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{image/prompting-format-v1.0.pdf}
    \caption{Prompting format of different tasks. \texttt{[Exemplars]} refer to the samples annotated with the correct answer from training set, keeping exactly the same format with the following input.}
    \label{fig:promp-format}
    \vspace{-0.2cm}
\end{figure*}

\section{Method}


% \subsection{Task Formulation}

% In this paper, we mainly focus on the logical reasoning of text tasks, which are formulated as multiple choice question answering. Specifically, given a context $C$, a question $Q$, and four options $\mathcal{O}=\{O_i\}$, the system should select the one best to address the question as the answer $A$. We also include the evaluation on BIG-Bench-Hard~\citep{big-bench-hard}, where most tasks give options, and others have free-form answers.

% \subsection{Prompting LLMs}

% \subsubsection{Zero-shot Prompting}

% For zero-shot prompting, the input to LLMs is as below:
% \begin{quote}
% \texttt{\small{Answer the following question based on the given context and options.}}

% \texttt{\small Context: \#$C$}

% \texttt{\small Question: \#$Q$}

% \texttt{\small Options:\\
% A: \#$O_0$. \\
% B: \#$O_1$. \\
% C: \#$O_2$. \\ 
% D: \#$O_3$. }

% \end{quote}.

% For zero-shot CoT prompting, we employed more detailed instructions to make sure LLMs could generate rationales:
% \begin{quote}
%     \texttt{\footnotesize You are shown a context, a question, and four options. Use logical reasoning capability to \textbf{analyze each option and select the best answer. Keep the output as concise as possible and think step by step.}}

%     \texttt{\small Context: \#$C$}

%     \texttt{\small Question: \#$Q$}
    
%     \texttt{\small Options:\\
%     A: \#$O_0$. \\
%     B: \#$O_1$. \\
%     C: \#$O_2$. \\ 
%     D: \#$O_3$. }
% \end{quote}

% \subsubsection{Few-shot Prompting}

% Denoting the zero-shot instruction as $I_z$ and zero-shot CoT instruction as $I_{zc}$, the inputs under zero-shot and zero-shot CoT setting can be simply represented as $[I_z, C, Q, \mathcal{O}]$ and $[I_{zc}, C, Q, \mathcal{O}]$, respectively. For vanilla few-shot prompting, we randomly select $n$ examples from the training set, add the correct option label using template \textit{The answer is $A$.}, and concatenate the examples after the instruction. For few-shot CoT, we replace the answer with the rationales, and LLMs are expected to first generate the rationales and finally reach the answer. The rationales of training set examples are automatically generated via zero-shot prompting LLMs, and we introduce self-consistency constraints to improve the quality of generated explanations by only keeping those reaching correct predictions. An example of few-shot CoT can be found in Figure~\ref{fig:few-shot-cot-exp}.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{image/chat-cot-example-v1-0.pdf}
%     \caption{An example chat-based prompting. \textit{Assistant} refers to the LLM. We omit the instruction at the very beginning.}
%     \label{fig:post-exp}
% \end{figure}

% \subsection{Post-prompting for Accurate Parsing}

% Since the output of LLMs via prompting are natural language, the regular approach to map the output into the space of option labels is by using the regular expression of Python through direct matching of the option index, i.e., A, B, C, and D.
% However, in the CoT setting, the style of response can be quite diverse, making it difficult to match the answer index.
% ChatGPT API supports \textit{chat} mode, in which the previous conversation history can serve as a prefix for a continual generation.
% Inspired by this, for each example with generated CoT, we concatenate a new prompt \textit{The answer is } afterwards to query the LLMs to repeat the final answer. The experimental results show that this trick could greatly improve the answer accuracy. An example is shown in Figure~\ref{fig:post-exp}.



\subsection{\meritp}

MERIt~\citep{merit} is a self-supervised pre-training method for logical reasoning, which achieves it by automatically constructing training samples for contrastive learning from Wikipedia documents. 
% The positive pair includes two logically consistent samples while the negative one does not. 
% Given an anchor entity pair, a positive instance describes a pair of logically consistent relations between these two entities, namely direct and indirect relations. And the negative instance is synthesized via relation replacement.
Given an arbitrary paragraph and an anchor entity pair \entpair{i}{j}, the \merit~framework first extracts a triplet \enttrip{i}{j} from the paragraph, where $r_{i,j}$ represents the relation between the entity pair $e_i$ and $e_j$.
In the original approach, $r_{i,j}$ could be any sentence in the paragraph that mentions \entpair{i}{j}, or specific relation annotated in an external knowledge base.
However, to ensure a fully self-supervised method, we only consider the intra-sentence relation triplet, \enttrips{i}{j}{k}, where $s_k$ is the sentence mentioning \entpair{i}{j}.
Additionally, we can find another sample with a chain of triplets, i.e., $\langle\, e_i, s_{i+1}, e_{i+1}, \cdots,s_{j},e_j\,\rangle$, which is viewed as an indirect relation between \entpair{i}{j}. This example pair is treated as a logically consistent instance.
To create a negative instance, we synthesize it by replacing \entpair{i}{j} into another sentence $s_t$ to replace the original entities.
By doing this, the framework treats logical reasoning of text as a composition of relations, avoiding reliance solely involving concise relation concepts defined in knowledge base.
Furthermore, to eliminate the information shortcut caused by the factual knowledge from LM pre-training, the framework also incorporates auto-generated counterfactual data via entity replacement mixed with a specific ratio. 
% It also comprises a counterfactual data augmentation strategy to enhance relation-centric reasoning.
In this paper, we omit additional details of data construction, and we refer readers to \citet{merit} for more details. Our main focus is on integrating the original contrastive learning objective into the training process of LLMs.

% Considering the downstream task-specific decoding strategy, we have explored two different integration approaches. For fine-tuning, since the downstream tasks also belong to text classification, we directly use the sequence-to-sequence architecture for contrastive learning, where the representation of the last token from decoder is extracted for similarity computation.
% For in-context learning, we have considered three different approaches. 

Given an anchor sample $x$ composed of a series of sentences, the logically consistent sample is denoted as $x^+$, and the negatively paired samples is represented as $\mathcal{X}^-$. The training objective for contrastive learning is formulated as:
\begin{equation}
    \begin{aligned}
    \mathcal{L}_{\mathrm{CL}}&=L(x, x^+, \mathcal{X}^-) \\
                             &=-\log\frac{\exp f(x, x^+)}{\sum_{x'\in\mathcal{X}^-\cup\{x^+\}}\exp f(x,x')},
                            % &=-\log\frac{\exp f(x, x^+)}{\exp f(x,x^+) + \exp f(x, x^-)},
    \end{aligned}
    \label{eqn:cl-obj}
\end{equation}
where $f(\cdot)$ is LLM taking the concatenation of $[x, x^+]$ or $[x, x^-]$ as input to compute the score. 
% In this paper, we employ an extra linear layer to map the representation of the \texttt{EOS} token in each input sequence into scalar space as the score.
Different from the conventional approach~\citep{bart}, where the representation of \texttt{EOS} token is employed for score computing, we employ a token-wise scoring implementation to contribute fine-grained optimization. The process can be formulated as
\begin{equation}
    \begin{aligned}
        f(x, x^+)=\frac{1}{|x'|}\sum_i^{|x|\le i\le |x|+|x'|} \mathbf{W}\mathbf{h}_i+\mathbf{b},
    \end{aligned}
\end{equation}
where $\mathbf{W}\in\mathbb{R}^{d\times 1}$ and $\mathbf{h}_i$ is the representation for the $i$-th token from the LLM.
% For the classification-based approach, i.e., fine-tuning, we employed a simple linear layer on the top of $f$ to map the representation of the last token in the sequence to compute the score. 
However, the contrastive learning based method could be unsuitable for LLM pre-training because it involves negative candidates and leads to exponential computation cost, which especially prolong the training time. 
To this end, we propose an auto-regressive variant by directly optimizing positive sequence, which is defined as:
\begin{equation}
\begin{aligned}
    \mathcal{L}_{\mathrm{AR}}&=-\log P(x^+|x) \\
                             &=-\sum_i^{|x^+|}\log P(x^+_i|x^+_{<i},x),
\end{aligned}
\end{equation}
where $x^+_i$ denotes the $i$-th token of $x^+$.
It should be noted that in this case, the carefully constructed negative samples are ignored, only the counterfactual data augmentation strategy of original MERIt works.


\subsection{LLM Prompting}
\label{sec:llm-prompting}

% In this paper, we tried 4 different settings for LLM prompting, i.e., zero-shot prompting, zero-shot CoT prompting, few-shot prompting, and few-shot CoT prompting. The input to LLMs can be formulated as 
% \begin{quote}
%     \texttt{\footnotesize{Instruction}} \\
%     \texttt{\footnotesize{[Exemplars]}} \\
%     \texttt{\footnotesize{Context: \#$C$}} \\
%     \texttt{\footnotesize{Question: \#$Q$}} \\
%     \texttt{\footnotesize{Options: \#$\mathcal{O}$}}.
% \end{quote}
% Specifically, [exemplars] are only used in few-shot settings. For vanilla few-shot prompting, each exemplar contains the context, question, options, and the response with the option index, e.g., \textit{The answer is Option A}. For few-shot CoT prompting, we also include the generated explanations. Considering the cost of manually annotation, we directly employed zero-shot CoT to generate seed explanations for each sample in the training set. After that, by checking if the predicted answer is consistent with the groundtruth one, the samples with reasonable auto-generated explanations can be kept as exemplar candidates. Besides, we to further improve the generalization of selected prompts, we also incorporate the reasoning category information. In Logiqa-V2, each question is also annotated with the reasoning category, e.g., categorical reasoning, sufficient conditional reasoning, and necessary conditional reasoning. During exemplar selection, only those sharing at least two common reasoning categories will serve as the candidates for few-shot CoT prompting.


In order to test the generalization across different tasks after post-training, we evaluate LLMs through prompting, where the input to LLMs can be formulated as \texttt{Instruction [Exemplars] Task input}. The instruction depends on specific task and exemplars are used only in few-shot setting. Each exemplar is composed by the task input and output. 
As shown in Figure~\ref{fig:promp-format}, for multiple choice question answering, the task input is the concatenation of the context, question and all options, with the correct option index as the output. 
In CoT setting, we also include the reasoning process in natural language between the task input and output.

Following \citet{mmlu2021}, during inference, for questions with candidate options, we enumerate each option to form different response template, e.g., \textit{The answer is D}. Then we can directly parse the prediction according to the last token probability instead of using regular expression. This is of great help to accelerate the evaluation process. For free-form answer and the evaluation of API-based model, e.g., ChatGPT, we still use regular expression to extract the answer from the generated content.
% \teng{method is too short}


==> backs/method-0617.tex <==
\input{figures/method}
% \input{figures/prompt-format}
\section{Method}

\subsection{\meritp}

The work by \merit~\citep{merit} introduces a self-supervised pre-training technique dedicated to improving logical reasoning. It accomplishes this by leveraging contrastive learning, which is a powerful tool used to automatically construct training samples from a corpus of Wikipedia documents. 

\noindent\textbf{Relation Representation.}
Given an arbitrary paragraph and an anchor entity pair \entpair{i}{j}, the \merit~framework first extracts a triplet \enttrip{i}{j} from the paragraph, where $r_{i,j}$ represents the \textbf{direct relation} between the entity pair $e_i$ and $e_j$.
% Conventionally, $r_{i,j}$ could be any sentence in the paragraph that mentions \entpair{i}{j}, or specific relation annotated in an external knowledge base.
Conventionally, $r_{i,j}$ includes both intra-sentence relation and the one annotated in knowledge base between \entpair{i}{j}.
To ensure the self-supervision of the method, in \merit, we restrict it only to the intra-sentence relation triplet, \enttrips{i}{j}{k}, in which $s_k$ is the sentence that mentions \entpair{i}{j}. After that, the framework can identify another example with a chain of triplets, such as $\langle e_i, s_{i+1}, e_{i+1}, \cdots,s_{j},e_j\rangle$. This is considered an \textbf{indirect relation} between \entpair{i}{j} and is treated as a logically consistent instance.

In terms of creating a negative instance, we synthesize it by replacing \entpair{i}{j} in another sentence $s_t$, hence substituting the original entities following \merit. The framework, thereby, converts the logical reasoning of text into a composition of relations. This is crucial because it prevents the process from relying solely on concise relation concepts defined in a knowledge base.

Moreover, to mitigate the information shortcut, which may arise from factual knowledge obtained from LM pre-training, the framework integrates auto-generated counterfactual data. This data is created by replacing entities and is mixed with a specific ratio to the original data.

In this paper, we refrain from providing additional details about data construction; we direct interested readers to \citet{merit} for comprehensive insights. Our primary focus remains on integrating the original contrastive learning objective into the training process of LLMs. Contrastive learning, in this context, plays a significant role. By leveraging contrasting positive (logically consistent instances) and negative (synthetic instances) samples, LogicLLM can better learn to differentiate between logically sound and unsound constructs. This process effectively sharpens the logical reasoning capabilities of LLMs.
% \jiao{I modified something here to keep anonymity. We cannot mention MERIt like the authors.}

In the context of our approach, an anchor sample $x$ is comprised of a series of sentences. A logically consistent sample is denoted as $x^+$, while the set of negatively paired samples is represented as $\mathcal{X}^-$. The objective for contrastive learning in this setting can be defined as: 
\begin{equation}
    \begin{aligned}
    \mathcal{L}_{\mathrm{CL}}&=L(x, x^+, \mathcal{X}^-) \\
                             &=-\log\frac{\exp f(x, x^+)}{\sum_{x'\in\mathcal{X}^-\cup\{x^+\}}\exp f(x,x')},
                            % &=-\log\frac{\exp f(x, x^+)}{\exp f(x,x^+) + \exp f(x, x^-)},
    \end{aligned}
    \label{eqn:cl-obj}
\end{equation}
where $f(\cdot)$ is LLM-based function taking the concatenation of $[x, x^+]$ or $[x, x^-]$ as input to compute the score. 

Different from the conventional approach~\citep{bart}, which uses the representation of the single ending \texttt{EOS} token for score computation, we employ a token-wise scoring implementation. This offers more granularity in optimization. The process can be mathematically formulated as:
\begin{equation}
    \begin{aligned}
        f(x, x^+)=\frac{1}{|x'|}\sum_i^{|x|\le i\le |x|+|x'|} \mathbf{W}_{x'_i}\mathbf{h}_i+\mathbf{b}_{x'_i},
    \end{aligned}
\end{equation}
where $\mathbf{W}_{x'_i}\in\mathbb{R}^{d\times 1}$ and $\mathbf{h}_i$ is the representation for the $i$-th token from the LLM, and $x'\in\mathcal{X}^-\cup\{x^+\}$. 
% \teng{What is $x'?$\jiao{Fixed}}

However, a contrastive learning-based method may not be ideal for LLM pre-training. This is because the inclusion of negative candidates results in an exponential computation cost, significantly increasing the training time. And a classification-based proxy task may hurt the in-context learning ability due to objective mismatch.
To address this issue, we propose an auto-regressive variant that directly optimizes the positive sequence. It is defined as:
% \teng{Only motivated from computation cost? Need to improve\jiao{Fixed}}
\begin{equation}
\begin{aligned}
    \mathcal{L}_{\mathrm{AR}}&=-\log P(x^+|x) \\
                             &=-\sum_i^{|x^+|}\log P(x^+_i|x^+_{<i},x),
\end{aligned}
\end{equation}
where $x^+_i$ denotes the $i$-th token of $x^+$.
It's worth noting that in this approach, the carefully constructed negative samples are disregarded. Instead, we rely solely on the counterfactual data augmentation strategy of the original MERIt framework.


\subsection{LLM Prompting}
\label{sec:llm-prompting}

In order to evaluate the generalization capabilities of LLMs across different tasks after post-training, we adopt a prompting-based approach. Here, the input to the LLMs is structured as \texttt{Instruction [Exemplars] Task input}. The instruction is tailored to the specific task at hand, while exemplars are utilized only in a few-shot setting. Each exemplar comprises both the task input and its corresponding output. As depicted in Figure~\ref{fig:promp-format}, for tasks such as multiple-choice question answering, the task input is a concatenation of the context, the question, and all potential options. The correct option index is used as the output. Besides, in a Chain-of-Thought (CoT) setting, we include a reasoning process formulated in natural language between the task input and output. 

% Following~\citet{mmlu2021}, during inference for questions with candidate options, we generate distinct response templates for each option. For instance, \textit{The answer is D}. By this means, we can parse the model's prediction directly based on the last token's probability, bypassing the need for regular expressions, which can significantly speed up the evaluation process.

% However, for free-form answers and when evaluating API-based models such as ChatGPT, we continue to employ regular expressions. These are necessary to accurately extract the answer from the content generated by the model.
% \teng{too much details here, The last 9 lines can be removed.}



==> backs/method0618.tex <==
\input{figures/method}
% \input{figures/prompt-format}
\section{Method}

\subsection{Meta-training}
% \subsection{\meritp}
\subsubsection{Relation Extraction}

As shown in Figure~\ref{fig:merit}, given an arbitrary paragraph and an anchor entity pair \entpair{i}{j}, we extract a triplet \enttrips{i}{j}{k} from the paragraph, where $s_k$ refers to some sentence directly mentioning \entpair{i}{j} and represents a \textbf{direct relation} between the entity pair.
Similarly, a chain of triplets, such as $\langle e_i, s_{i+1}, e_{i+1}, \cdots,s_{j},e_j\rangle$, can be identified and treated as an \textbf{indirect relation} between \entpair{i}{j}.
Intuitively, the two relations between \entpair{i}{j} should be logically consistent~\citep{merit} since they are derived from same context.
Unlike \citet{merit}, we did not include the relation annotated external knowledge base. This will waive the chance to incorporate commonsense knowledge, but can ensure the fully self-supervised nature.
% Conventionally, $r_{i,j}$ includes both intra-sentence relation and the one annotated in knowledge base between \entpair{i}{j}.
% To ensure the self-supervision of the method, in \merit, we restrict it only to the intra-sentence relation triplet, \enttrips{i}{j}{k}, in which $s_k$ is the sentence that mentions \entpair{i}{j}. 

% The work by \merit~\citep{merit} introduces a self-supervised pre-training technique dedicated to improving logical reasoning. It accomplishes this by leveraging contrastive learning, which is a powerful tool used to automatically construct training samples from a corpus of Wikipedia documents. 

\subsubsection{Auto-regressive Generative Training}

Dedicated to in-context learning, we consider integrating the relation reconstruction task with the auto-regressive generation. As illustrated in Figure~\ref{fig:merit}, taking either example from a logically consistent pair as the condition, the LLM is expected to minimize the log-likelihood of the other side, which is formulated as:
\begin{equation}
\begin{aligned}
    \mathcal{L}_{\mathrm{AR}}&=-\log P(x^+|x) \\
                             &=-\sum_i^{|x^+|}\log P(x^+_i|x^+_{<i},x),
\end{aligned}
\end{equation}
where $x^+_i$ denotes the $i$-th token of $x^+$.


\subsubsection{Counterfactual Data Augmentation}

Though the implementation of auto-regressive generative training is simple, it can be more possible to be mislead to memorization instead of logical reasoning.
Taking a corner case as example, when the logically consistent instance pair has covered all the sentences in the paragraph, the self-supervised task is then degraded into simple paragraph completion by recovering the compressed knowledge from the pre-training stage.
To this end, we employ similar counterfactual data augmentation strategy with \citet{merit}.
A set of new entities is sampled from an paragraph belonging to another document to replace the entities composing the logical chain in the original example.
This enables entity-irrelevant reasoning, making LLM more focused on the relational composition process.

% \noindent\textbf{Relation Representation.}
% Given an arbitrary paragraph and an anchor entity pair \entpair{i}{j}, the \merit~framework first extracts a triplet \enttrip{i}{j} from the paragraph, where $r_{i,j}$ represents the \textbf{direct relation} between the entity pair $e_i$ and $e_j$.
% % Conventionally, $r_{i,j}$ could be any sentence in the paragraph that mentions \entpair{i}{j}, or specific relation annotated in an external knowledge base.
% Conventionally, $r_{i,j}$ includes both intra-sentence relation and the one annotated in knowledge base between \entpair{i}{j}.
% To ensure the self-supervision of the method, in \merit, we restrict it only to the intra-sentence relation triplet, \enttrips{i}{j}{k}, in which $s_k$ is the sentence that mentions \entpair{i}{j}. After that, the framework can identify another example with a chain of triplets, such as $\langle e_i, s_{i+1}, e_{i+1}, \cdots,s_{j},e_j\rangle$. This is considered an \textbf{indirect relation} between \entpair{i}{j} and is treated as a logically consistent instance.

% In terms of creating a negative instance, we synthesize it by replacing \entpair{i}{j} in another sentence $s_t$, hence substituting the original entities following \merit. The framework, thereby, converts the logical reasoning of text into a composition of relations. This is crucial because it prevents the process from relying solely on concise relation concepts defined in a knowledge base.

% Moreover, to mitigate the information shortcut, which may arise from factual knowledge obtained from LM pre-training, the framework integrates auto-generated counterfactual data. This data is created by replacing entities and is mixed with a specific ratio to the original data.

% In this paper, we refrain from providing additional details about data construction; we direct interested readers to \citet{merit} for comprehensive insights. Our primary focus remains on integrating the original contrastive learning objective into the training process of LLMs. Contrastive learning, in this context, plays a significant role. By leveraging contrasting positive (logically consistent instances) and negative (synthetic instances) samples, LogicLLM can better learn to differentiate between logically sound and unsound constructs. This process effectively sharpens the logical reasoning capabilities of LLMs.
% % \jiao{I modified something here to keep anonymity. We cannot mention MERIt like the authors.}

% In the context of our approach, an anchor sample $x$ is comprised of a series of sentences. A logically consistent sample is denoted as $x^+$, while the set of negatively paired samples is represented as $\mathcal{X}^-$. The objective for contrastive learning in this setting can be defined as: 
% \begin{equation}
%     \begin{aligned}
%     \mathcal{L}_{\mathrm{CL}}&=L(x, x^+, \mathcal{X}^-) \\
%                              &=-\log\frac{\exp f(x, x^+)}{\sum_{x'\in\mathcal{X}^-\cup\{x^+\}}\exp f(x,x')},
%                             % &=-\log\frac{\exp f(x, x^+)}{\exp f(x,x^+) + \exp f(x, x^-)},
%     \end{aligned}
%     \label{eqn:cl-obj}
% \end{equation}
% where $f(\cdot)$ is LLM-based function taking the concatenation of $[x, x^+]$ or $[x, x^-]$ as input to compute the score. 

% Different from the conventional approach~\citep{bart}, which uses the representation of the single ending \texttt{EOS} token for score computation, we employ a token-wise scoring implementation. This offers more granularity in optimization. The process can be mathematically formulated as:
% \begin{equation}
%     \begin{aligned}
%         f(x, x^+)=\frac{1}{|x'|}\sum_i^{|x|\le i\le |x|+|x'|} \mathbf{W}_{x'_i}\mathbf{h}_i+\mathbf{b}_{x'_i},
%     \end{aligned}
% \end{equation}
% where $\mathbf{W}_{x'_i}\in\mathbb{R}^{d\times 1}$ and $\mathbf{h}_i$ is the representation for the $i$-th token from the LLM, and $x'\in\mathcal{X}^-\cup\{x^+\}$. 
% % \teng{What is $x'?$\jiao{Fixed}}

% However, a contrastive learning-based method may not be ideal for LLM pre-training. This is because the inclusion of negative candidates results in an exponential computation cost, significantly increasing the training time. And a classification-based proxy task may hurt the in-context learning ability due to objective mismatch.
% To address this issue, we propose an auto-regressive variant that directly optimizes the positive sequence. It is defined as:
% % \teng{Only motivated from computation cost? Need to improve\jiao{Fixed}}
% \begin{equation}
% \begin{aligned}
%     \mathcal{L}_{\mathrm{AR}}&=-\log P(x^+|x) \\
%                              &=-\sum_i^{|x^+|}\log P(x^+_i|x^+_{<i},x),
% \end{aligned}
% \end{equation}
% where $x^+_i$ denotes the $i$-th token of $x^+$.
% It's worth noting that in this approach, the carefully constructed negative samples are disregarded. Instead, we rely solely on the counterfactual data augmentation strategy of the original MERIt framework.


\subsubsection{Training}

During training, we fix the ratio between normal data and counterfactual data as 1:3 and do not change it. Following \citet{merit}, we add the original causal language modeling loss on Wikipedia corpus to avoid the catastrophic forgetting problem. The overall training objective is defined as:
\begin{equation}
    \mathcal{L}=\mathcal{L}_{AR}+\mathcal{L}_{LM}.
\end{equation}

\subsection{LLM Prompting}
\label{sec:llm-prompting}

In order to evaluate the generalization capabilities of LLMs across different tasks after post-training, we adopt a prompting-based approach. Here, the input to the LLMs is structured as \texttt{Instruction [Exemplars] Task input}. The instruction is tailored to the specific task at hand, while exemplars are utilized only in a few-shot setting. Each exemplar comprises both the task input and its corresponding output. For tasks such as multiple-choice question answering, the task input is a concatenation of the context, the question, and all potential options. The correct option index is used as the output. Besides, in a Chain-of-Thought (CoT) setting, we include a reasoning process formulated in natural language between the task input and output. 

% Following~\citet{mmlu2021}, during inference for questions with candidate options, we generate distinct response templates for each option. For instance, \textit{The answer is D}. By this means, we can parse the model's prediction directly based on the last token's probability, bypassing the need for regular expressions, which can significantly speed up the evaluation process.

% However, for free-form answers and when evaluating API-based models such as ChatGPT, we continue to employ regular expressions. These are necessary to accurately extract the answer from the content generated by the model.
% \teng{too much details here, The last 9 lines can be removed.}



==> backs/sec5.2.tex <==
\subsection{General Language Understanding}
% \jiao{Remove DREAM results of FLAN-T5 series due to marginal improvements and non-zero-shot testing. We may need new datasets, e.g., RACE, MMLU.}
Beside logical reasoning of text, we also care about whether the logic-enhanced training contributes to general language understanding. To this end, we evaluate the enhanced \llama~models on RACE and MMLU. 
% For FLAN-T5 series, we find that the grades are nearly saturated, possibly because FLAN-collection has already included many reading comprehension and reasoning datasets. As a result, the improvements brought by MERIt are marginal.
% We omit the results of \flant~series models because DREAM is already included in FLAN collection and they are not zero-shot test. The results can be found in Appendix~\ref{}.
As shown in Table~\ref{tab:dream}, \llama~w/ MERIt makes significant improvements compared with the baseline on RACE. The improvements on MMLU are relatively limited considering most tasks require domain specific knowledge, which can be hard compressed in smaller models. We also show the detailed results on each sub-task in Table~\ref{tab:mmlu-detail}. 
% And we can also find that the enhanced 7B model can perform comparable with \llama-13B on the validation set of DREAM, demonstrating the effectiveness of the proposed method.
% However, on LLaMA series, the improvements are really significant. And the margin also increases when scaled the parameters are scaled from 7 billion to 13 billion, demonstrating the effectiveness and generalization of logic-enhanced training for LLMs.

Additionally, we also evaluate the performance of trained models on BIG-Bench-Hard, a benchmark composed of multiple challenging tasks where human still performs much better than LLMs. From Table~\ref{tab:bbh} we can conclude that 
(1) \merit~enhances the performance under both zero-shot setting and direct few-shot setting, suggesting that logic-enhanced training also improves the performance on the complex reasoning tasks. 
% (2) Logic-enhance training can be well integrated with instruction tuning. Benefiting FLAN collection, the improvements are consistent on both \flant-3B and \flant-11B models.
(2) Few-shot prompting, including both \textit{direct} and \textit{CoT} setting, cannot make significant improvements compared with that under zero-shot setting, except for \llama. This is because some questions have free-formed answers, and \llama~can hardly stop generating without exemplars.


==> backs/sec5.5.tex <==
Table~\ref{tab:cot} presents the evaluation of LLMs' performance in few-shot and CoT settings. The intermediate reasoning process is generated automatically by ChatGPT using the prompt \textit{Let's think step by step}. In the case of zero-shot CoT, we append the suffix prompt - \textit{So the answer is} to guide the models in summarizing and concluding the answer. For few-shot CoT, the reasoning process is initially generated for each sample in the training set. Subsequently, we retain the samples where the final prediction is correct, following the steps in zero-shot CoT.
During testing, we randomly select samples from the retained candidates, as well as the automatically generated CoT, to serve as exemplars. However, we observe that both few-shot learning and using CoT do not significantly benefit the models. One possible reason is that the selected samples differ greatly from the target example. To verify this, we include the reasoning category information during exemplar selection. In LogiQA-V2, each question is annotated with a reasoning category such as categorical reasoning, sufficient conditional reasoning, and necessary conditional reasoning. For few-shot CoT prompting, we only consider candidates that share at least two common reasoning categories. This method variant is denoted as \textit{ChatGPT w/ CoT + Cate.} in the table.
Nevertheless, we find that carefully selecting prompting exemplars also provides limited improvement. All the results indicate that LLMs struggle to grasp the reasoning structure from a limited number of observed examples. Consequently, they are unable to learn the mapping between input-label and input-rationale-label effectively. Additionally, we can observe from Table~\ref{tab:logic} that \meritp~also contributes little to addressing this problem. We leave further investigation of this matter to future work.

==> backs/tables/main_res.tex <==
% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{2.5mm}{
% \scalebox{0.9}{
% \begin{tabular}{l|c|cc|cc|cc}
% % \hline
% \toprule
%       &                 & \multicolumn{2}{c}{\textbf{ReClor}}  & \multicolumn{2}{|c}{\textbf{LogiQA}} & \multicolumn{2}{|c}{\textbf{LogiQA-v2}} \\
% Model / Dataset         & Training     & Dev         & Test       & Dev     & Test    & Dev     & Test \\
%                         &              & Acc.        & Acc.       & Acc.    & Acc.    & Acc.    & Acc.     \\ \hline
% \rob-L.                 &  FT          & 62.6        & 55.6       & 35.0    & 35.3    & 59.8  & 57.0       \\
% MERIt                   &  FT          & \tb{69.4}   & 61.6       & 39.9    & 40.7    & 62.6  & 59.3   \\
% MERIt*                  &  FT          & 68.5        & 62.7       &         &         & 62.6  & 59.2   \\ 
% DeBERTa-v2-1.5B         &  FT          & 78.3        & 75.3       &         &         & 62.6  & 59.2   \\ \hline
% GPT-3.5-turbo (0-shot)  &  ICL         & 61.8        &            &         &         & 54.5  &           \\ 
% ~~w/ CoT (0-shot)       &  ICL         & 50.2        &            &         &         &       &           \\ \hline
% FLAN-T5-3B              &  FT          & 79.7        & 75.7       &         &         &       &           \\  
% ~~w/ MERIt              &  FT          & 79.6        & \textbf{76.2}  &         &         &       &             \\ \hline
% FLAN-T5-3B (0-shot)     &  ICL         & 54.6        &            &         &         & 48.7  &           \\
% ~~w/ CoT (o-shot)       &  ICL         & 54.6        &            &         &         & 48.5  &           \\
% FLAN-T5-3B (1-shot)     &  ICL         & 55.6        &            &         &         & 55.6  &           \\
% FLAN-T5-3B (3-shot)     &  ICL         & 56.4        &            &         &         & 56.2  &           \\ \hline
% FLAN-T5-11B (0-shot)    &  ICL         & 57.2        &            &         &         & 55.9  &           \\  
% ~~w/ CoT (0-shot)       &  ICL         & 56.0        &            &         &         & 54.6  &           \\  
% \bottomrule
% \end{tabular}
% }}
% \caption{\textbf{FT}: Fine-tuning. \textbf{ICL}: In-Context Learning.}
% % \vspace{-0.3cm}
% \label{tab:mcqa}
% \end{table*}

% ====================================================


% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{3.2mm}{
% \scalebox{0.9}{
% \begin{tabular}{lccccccc}
% % \hline
% \toprule
%       &                 & \multicolumn{2}{c}{\textbf{ReClor}}  & \multicolumn{2}{c}{\textbf{LogiQA-v2}} & \multicolumn{2}{c}{\textbf{DREAM}}\\
% Model / Dataset         & Training     & Dev         & Test             & Dev     & Test        & Dev     & Test    \\
%                         &              & Acc.        & Acc.             & Acc.    & Acc.        & Acc.    & Acc.    \\ \hline
% % \rob-L.                 &  FT          & 62.6        & 55.6             & 59.8  & 57.0          &           &           \\
% % MERIt                   &  FT          & \tb{69.4}   & 61.6             & 62.6  & 59.3          &           &           \\
% % MERIt*                  &  FT          & 68.5        & 62.7             & 62.6  & 59.2          &           &           \\ 
% % DeBERTa-v2-1.5B         &  FT          & 78.3        & 75.3             & 62.6  & 59.2          &           &           \\ \hline
% % FLAN-T5-3B              &  FT          & 79.7        & 75.7             & 72.9  & 70.2          &           &           \\  
% % ~~w/ MERIt              &  FT          & \bf{80.2}   & \textbf{76.2}    & 73.0  & 69.9          &           &            \\ \hline
% \textit{zero-shot} \\ \hline
% ChatGPT                 &  ICL         & 56.6        & 61.2             & 54.5  & 52.7          & 89.5      & 90.4          \\ 
% ~~~~w/ CoT              &  ICL         & 58.8        & 57.7             & 54.5   & 53.1         &           &               \\ \hline
% FLAN-T5-3B              &  ICL         & 54.6        & 52.5             & 48.7  & 48.7          & 91.0      & 93.1 \\
% ~~~~w/ FLAN             &  ICL         & 53.6        & 53.8             & 49.5  & 49.5          & 91.1      & 92.1  \\
% % ~~w/ MERIt (\textit{ctr} ) & ICL       &             &                  \\
% % ~~w/ MERIt + FLAN (\textit{ctr}) & ICL & 54.6        & 52.5             &            & 48.8      \\
% ~~~~w/ MERIt + FLAN     &   ICL        & \bf{55.8}   & \bf{54.1}        & \bf{50.8}   & \bf{50.1}& \bf{91.7} & 92.1   \\ 
% FLAN-T5-11B             &  ICL         & 57.4        & 59.9             & 55.3        & 53.1     & 93.0     & 94.1 \\  
% ~~~~w/ FLAN             &  ICL         & 58.0        & 60.5             & \bf{56.9}   & 53.6     & 93.2     & 94.1  \\
% ~~~~w/ MERIt + FLAN     & ICL          & \bf{61.2}   & \bf{61.1}        & 56.0        & \bf{54.0}& \bf{93.5}& \bf{94.3} \\  \hline
% \llama-7B               & 28.8         & 28.3        & 24.4             & 23.7        & 42.0     & 42.6      \\
% ~~w/ \merit             & 27.8         & \bf{29.4}   & \bf{28.0}        & \bf{29.3}   & \bf{50.2}& \bf{51.0}  \\ % 100 step
% ~~w/ \merit~(ctr)       & \bf{31.2}    &             & \bf{29.2}        & \bf{29.6}   & \bf{53.0}& \bf{52.4} \\ % 500 step \hline 
% \llama-13B              & 31.6         & 34.4        & 31.6             & 31.1        & 50.3     & 55.0            \\
% ~~w/ \merit             & \bf{34.6}    & \bf{36.7}   & \bf{35.0}        & \bf{34.3}   & \bf{66.6}& \bf{68.7}   \\ % 100 step 
% \textit{3-shot} \\ \hline
% FLAN-T5-3B              &  ICL         & 50.3       &  49.1             & 50.3  &  49.1        & 91.7      & 92.5 \\
% ~~~~w/ FLAN             &  ICL         & 54.8       &  53.0             & 49.7  & 49.1         & 90.6      & 91.9 \\ % step 200
% % ~~w/ MERIt + FLAN (\textit{ctr}) & ICL & 54.6        & 52.5             &       & 48.8      \\
% ~~~~w/ MERIt + FLAN (\textit{ar})& ICL & \bf{56.2}  &  \bf{54.5}        & \bf{50.6}  & \bf{50.3} & 91.3    & \bf{92.9}    \\ \hline
% % \textit{3-shot CoT (generated by ChatGPT)} \\ \hline
% % FLAN-T5-3B      &  ICL         &         &              &   &           \\
% % ~~w/ FLAN               &  ICL         &        &          & 48.9  &        \\
% % ~~w/ MERIt + FLAN (\textit{ar})  & ICL &   &         & 49.0  &     \\
% % FLAN-T5-3B (1-shot)     &  ICL         & 55.6        &                  & 55.6  &           \\
% % FLAN-T5-3B (3-shot)     &  ICL         & 56.4        &                  & 56.2  &           \\ \hline
% \bottomrule
% \end{tabular}
% }}
% \caption{The results of FLAN-T5 series on multiple choice reasoning benchmarks comapred with ChatGPT. \textbf{FT}: Fine-tuning. \textbf{ICL}: In-Context Learning.}
% % \vspace{-0.3cm}
% \label{tab:mcqa}
% \end{table*}


\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4.0mm}{
\scalebox{0.9}{
\begin{tabular}{lcccccc}
% \hline
\toprule
                        & \multicolumn{2}{c}{\textbf{ReClor}}  & \multicolumn{2}{c}{\textbf{LogiQA-v2}} & \multicolumn{2}{c}{\textbf{DREAM}}\\
Model / Dataset         & Dev         & Test             & Dev     & Test        & Dev     & Test    \\
                        & Acc.        & Acc.             & Acc.    & Acc.        & Acc.    & Acc.    \\ \hline
% \rob-L.                 &  FT          & 62.6        & 55.6             & 59.8  & 57.0          &           &           \\
% MERIt                   &  FT          & \tb{69.4}   & 61.6             & 62.6  & 59.3          &           &           \\
% MERIt*                  &  FT          & 68.5        & 62.7             & 62.6  & 59.2          &           &           \\ 
% DeBERTa-v2-1.5B         &  FT          & 78.3        & 75.3             & 62.6  & 59.2          &           &           \\ \hline
% FLAN-T5-3B              &  FT          & 79.7        & 75.7             & 72.9  & 70.2          &           &           \\  
% ~~w/ MERIt              &  FT          & \bf{80.2}   & \textbf{76.2}    & 73.0  & 69.9          &           &            \\ \hline
\textit{zero-shot} \\ \hline
ChatGPT                 & 56.6        & 61.2             & 54.5  & 52.7          & 89.5      & 90.4          \\ 
~~~~w/ CoT              & 58.8        & 57.7             & 54.5   & 53.1         & 81.7      & 81.5          \\ \hline
\llama-7B               & 28.8        & 28.3        & 24.4             & 23.7        & 42.0     & 42.6      \\
~~~~w/ \merit             & 27.8        & \bf{29.4}   & \bf{28.0}        & \bf{29.3}   & \bf{50.2}& \bf{51.0}  \\ % 100 step
%%~~~~w/ \merit~(ctr)       & \bf{31.2}   & \bf{31.1}   & \bf{29.2}        & \bf{29.6}   & \bf{53.0}& \bf{52.4} \\ % 500 step \hline  %save for next version 2023-05-20 
\hdashline
\llama-13B              & 31.6        & 34.4        & 31.6             & 31.1        & 50.3     & 55.0            \\
~~~~w/ \merit             & \bf{34.6}   & \bf{36.7}   & \bf{35.0}        & \bf{34.3}   & \bf{66.6}& \bf{68.7}   \\ % 100 step 
\hline 
FLAN-T5-3B              & 54.6        & 52.5             & 48.7  & 48.7          & 91.0      & 93.1 \\
%%#% ~~~~w/ FLAN             & 53.6        & 53.8             & 49.5  & 49.5          & 91.1      & 92.1  \\
% ~~w/ MERIt (\textit{ctr} ) & ICL       &             &                  \\
% ~~w/ MERIt + FLAN (\textit{ctr}) & ICL & 54.6        & 52.5             &            & 48.8      \\
~~~~w/ MERIt + FLAN     & \bf{55.8}   & \bf{54.1}        & \bf{50.8}   & \bf{50.1}& \bf{91.7} & 92.1   \\ 
  \hdashline
FLAN-T5-11B             & 57.4        & 59.9             & 55.3        & 53.1     & 93.0     & 94.1 \\  
%%#% ~~~~w/ FLAN             & 58.0        & 60.5             & \bf{56.9}   & 53.6     & 93.2     & 94.1  \\
~~~~w/ MERIt + FLAN     & \bf{61.2}   & \bf{61.1}        & \bf 56.0        & \bf{54.0}& \bf{93.5}& \bf{94.3} \\  \hline

\textit{3-shot} \\ \hline
FLAN-T5-3B              & 50.3       &  49.1             & 50.3  &  49.1        & 91.7      & 92.5 \\
%%#% ~~~~w/ FLAN             & 54.8       &  53.0             & 49.7  & 49.1         & 90.6      & 91.9 \\ % step 200
% ~~w/ MERIt + FLAN (\textit{ctr}) & ICL & 54.6        & 52.5             &       & 48.8      \\
~~~~w/ MERIt + FLAN \iffalse (\textit{ar})\fi & \bf{56.2}  &  \bf{54.5}        & \bf{50.6}  & \bf{50.3} & 91.3    & \bf{92.9}    \\ 
% \textit{3-shot CoT (generated by ChatGPT)} \\ \hline
% FLAN-T5-3B      &  ICL         &         &              &   &           \\
% ~~w/ FLAN               &  ICL         &        &          & 48.9  &        \\
% ~~w/ MERIt + FLAN (\textit{ar})  & ICL &   &         & 49.0  &     \\
% FLAN-T5-3B (1-shot)     &  ICL         & 55.6        &                  & 55.6  &           \\
% FLAN-T5-3B (3-shot)     &  ICL         & 56.4        &                  & 56.2  &           \\ \hline
\bottomrule
\end{tabular}
}}
\caption{The results of FLAN-T5 and LLaMA series on multiple choice reasoning benchmarks compared with ChatGPT. Better results are annotated in bold.}
% \vspace{-0.3cm}
\label{tab:mcqa}
\end{table*}

% ====================================================


% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{2.5mm}{
% \scalebox{0.85}{
% \begin{tabular}{lccc}
% % \hline
% \toprule
%       &                 & \multicolumn{2}{c}{\textbf{ReClor}}       \\
% Model / Dataset         & Training     & Dev         & Test         \\
%                         &              & Acc.        & Acc.               \\ \hline
% % \textit{fine-tuning} \\ \hline
% \rob-L.                 &  FT          & 62.6        & 55.6                 \\
% MERIt                   &  FT          & \tb{69.4}   & 61.6           \\
% MERIt*                  &  FT          & 68.5        & 62.7        \\ 
% DeBERTa-v2-1.5B         &  FT          & 78.3        & 75.3           \\ \hline
% FLAN-T5-3B              &  FT          & 79.7        & 75.7              \\  
% ~~w/ MERIt              &  FT          & \bf{80.2}   & \textbf{76.8}          \\ \hline
% % \textit{prompting} \\ \hline
% GPT-3.5-turbo           &  ICL         & 56.6        & 61.2               \\ 
% ~~w/ CoT                &  ICL         & 58.8        & 57.7          \\ \hline
% FLAN-T5-3B              &  ICL         & 54.6        & 52.5                   \\
% ~~w/ FLAN               &  ICL         & 53.6        & 53.8              \\
% % ~~w/ MERIt (\textit{ctr} ) & ICL       &             &                  \\
% ~~w/ MERIt + FLAN (\textit{ctr}) & ICL & 54.6        & 52.5         \\
% ~~w/ MERIt + FLAN (\textit{ar})  & ICL & \bf{55.8}   & \bf{54.1}             \\
% % FLAN-T5-3B (1-shot)     &  ICL         & 55.6        &                   \\
% % FLAN-T5-3B (3-shot)     &  ICL         & 56.4        &                      \\ \hline
% % FLAN-T5-11B (0-shot)    &  ICL         & 57.2        &                     \\  
% \bottomrule
% \end{tabular}
% }}
% \caption{\textbf{FT}: Fine-tuning. \textbf{ICL}: In-Context Learning.}
% % \vspace{-0.3cm}
% \label{tab:mcqa}
% \end{table}

\iffalse 
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4.0mm}{
\scalebox{0.9}{
\begin{tabular}{lccccccc}
% \hline
\toprule
                        & \multicolumn{2}{c}{\textbf{ReClor}}  & \multicolumn{2}{c}{\textbf{DREAM}} & \multicolumn{1}{c}{\textbf{BIG-Bench-Hard}}\\
Model / Dataset         & Dev         & Test             & Dev     & Test        & Test     & Direct  &  CoT  \\
                        & Acc.        & Acc.             & Acc.    & Acc.        & Acc.    & Acc.  & Acc.    \\ \hline
FLAN-T5-3B              & 54.6        & 52.5               & 91.0      & 93.1 & 38.0        & 40.2       & 13.3        \\
 ~~~~w/ FLAN             & 53.6        & 53.8                      & 91.1      & 92.1  & 39.8        & 40.5       & 0.0  \\
~~~~w/ MERIt + FLAN     & \bf{55.8}   & \bf{54.1}        &  \bf{91.7} & 92.1 & \bf{40.5}   & \bf{41.2}  & \bf{16.8}  \\ 
  \hdashline
FLAN-T5-11B             & 57.4        & 59.9              & 93.0     & 94.1 & 43.0        & 42.6       & 40.9 \\  
 ~~~~w/ FLAN             & 58.0        & 60.5                 & 93.2     & 94.1 & 43.1        & 32.1       & 40.6  \\
~~~~w/ MERIt + FLAN     & \bf{61.2}   & \bf{61.1}        & \bf{93.5}& \bf{94.3}  & \bf{44.1}   & 36.2       & 40.2  \\  
\bottomrule
\end{tabular}
}}
\caption{Ablation study.}
% \vspace{-0.3cm}
\label{tab:mcqa}
\end{table*}
\fi 

\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4.0mm}{
\scalebox{0.9}{
\begin{tabular}{lccccccc}
% \hline
\toprule
                        & \multicolumn{2}{c}{\textbf{ReClor}}  & \multicolumn{2}{c}{\textbf{DREAM}} & \multicolumn{1}{c}{\textbf{BIG-Bench-Hard}}\\
Model / Dataset         & Dev         & Test             & Dev     & Test        & Test       \\
                        & Acc.        & Acc.             & Acc.    & Acc.        & Acc.       \\ \hline
FLAN-T5-3B              & 54.6        & 52.5               & 91.0      & 93.1 & 38.0              \\
 ~~~~w/ FLAN             & 53.6        & 53.8                      & 91.1      & 92.1  & 39.8         \\
~~~~w/ MERIt + FLAN     & \bf{55.8}   & \bf{54.1}        &  \bf{91.7} & 92.1 & \bf{40.5}     \\ 
  \hdashline
FLAN-T5-11B             & 57.4        & 59.9              & 93.0     & 94.1 & 43.0         \\  
 ~~~~w/ FLAN             & 58.0        & 60.5                 & 93.2     & 94.1 & 43.1         \\
~~~~w/ MERIt + FLAN     & \bf{61.2}   & \bf{61.1}        & \bf{93.5}& \bf{94.3}  & \bf{44.1}   \\  
\bottomrule
\end{tabular}
}}
\caption{Ablation study.}
% \vspace{-0.3cm}
\label{tab:mcqa}
\end{table*}

==> figures/pre-exp.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{image/preliminary_image_v1_4.pdf}
    \caption{The test set accuracy of LLaMA models with parameter sizes of 7B, 13B, and 33B, ChatGPT, Roberta-Large and the state-of-the-art method MERIt~\cite{merit} on two logical reasoning benchmarks, ReClor and LogiQA-v2. 
    % \teng{Can you remove the unnecessary blank space of the png file below acc using inkscape?}}
    }
    \vspace{-0.2cm}
    \label{fig:pre-exp}
    % \vspace{-1em}
\end{figure}

==> figures/prompt-format.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.98\linewidth]{image/prompting-format-v1.0.pdf}
    \caption{Prompting format of different tasks. \texttt{[Exemplars]} refer to the samples annotated with the correct answer from training set, keeping exactly the same format with the following input.}
    \label{fig:promp-format}
    \vspace{-0.2cm}
\end{figure*}



==> rebuttal/rebuttal.tex <==

Main concern of different reviewers:

Theoretical connection between relation discrimination and logical reasoning:
1. The direct relation and indirect relation may not be (logically) consistent in the same paragraph.
    1.1 Reviewer ZXV6 suggests adding statistical analysis about the assumption (how often it happens) or providing more constraints.
    1.2 Reviewer qK7f gives an example to refute this.
2. The pre-training method is not relevant to logical reasoning.
    2.1 The terminology from formal reasoning is confusing. (@Reviewer qk7f)

Counterfactual data may lead to extra noise.
1. Our method treat normal data and counterfactual data equally (@Reviewer qk7f)

Other concern:
1. Marginal improvements
RE: I think the improvements have been eoungh. We need to clarify the setting (fully self-supervised).

2. Necessity (instruction tuning seems more useful)
RE: We need to clarify recent instruction tuning is indeed knowledge distillation. It's unfair. We can update the results between Llama2 and Llama2-chat to show the effects of instruction tuning.

3. Difference with MERIt.
RE: Auto-regressive training strategy.




==> tables/bbh-detail.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{2.5mm}{
\scalebox{0.9}{
\begin{tabular}{lcccc}
% \hline
\toprule
                        & \multicolumn{3}{c}{\textbf{FLAN-T5-3B + }}  & \multicolumn{2}{c}{\textbf{LogiQA-v2}} \\
Model / Dataset         & Dev         & Test          & Dev     & Test \\
                        & Acc.        & Acc.          & Acc.    & Acc.     \\ \hline
\textit{0-shot} \\ \hline
ChatGPT                 & 56.6        & 61.2          & 54.5    & 52.7      \\ 
~~w/ CoT                & 58.8        & 57.7          & 54.5    & 53.1      \\ \hline
\textit{5-shot}  \\ \hline
ChatGPT           & 61.0        & \textbf{63.0} & 55.07   & 54.5      \\
~~w/ CoT              & \bf{62.0}   & 62.5 & 47.56   & \bf{55.6}   \\
~~w/ CoT + Cate.      &  N/A        & N/A           & \bf{55.8}& 55.0           \\
\bottomrule
\end{tabular}
}}
\caption{The results on logical reasoning benchmarks with enhanced Chain-of-Thought prompting.}
\label{tab:cot}
\end{table*}

==> tables/llama_main.tex <==
% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{3.2mm}{
% \scalebox{0.9}{
% \begin{tabular}{lccccccccc}
% % \hline
% \toprule
%                & \multicolumn{2}{c}{\textbf{ReClor}}  & \multicolumn{2}{c}{\textbf{LogiQA-v2}} & \multicolumn{2}{c}{\textbf{DREAM}} & \multicolumn{3}{c}{\textbf{BIG-Bench-Hard}} \\
% Model / Dataset         & Dev         & Test      & Dev      & Test        & Dev      & Test      & Zero-shot & Direct & CoT \\
%                         & Acc.        & Acc.      & Acc.     & Acc.        & Acc.     & Acc.      & Acc.        & Acc.        & Acc.  \\ \hline
% \llama-7B               & 28.8        & 28.3      & 24.4     & 23.7        & 42.0     & 42.6      & 24.9        & 30.4        & 27.0\\
% ~~w/ \merit             & 27.8        & \bf{29.4} & \bf{28.0}& \bf{29.3}   & \bf{50.2}& \bf{51.0} & \bf{25.2}   & \bf{30.8}        & 25.9 \\ % 100 step
% ~~w/ \merit~(ctr)       & \bf{31.2}   &           & \bf{29.2}& \bf{29.6}   & \bf{53.0}& \bf{52.4} &             &             &  \\ % 500 step \hline 
% \llama-13B              & 31.6        & 34.4      & 31.6     & 31.1        & 50.3     & 55.0     & 25.0        & 34.7        & 32.3        \\
% ~~w/ \merit             & \bf{34.6}   & \bf{36.7} & \bf{35.0}& \bf{34.3}   & \bf{66.6}& \bf{68.7} & \bf{26.3}   & \bf{35.0}   & \bf{33.9}   \\ % 100 step 
% \bottomrule
% \end{tabular}
% }}
% \caption{Results of \llama~with \merit~ on multiple choice reasoning benchmarks.}
% % \vspace{-0.3cm}
% \label{tab:llama-main}
% \end{table*}



==> tables/mmlu.tex <==
% llama-7b + MERIt (ar) step 250
% {"overall_acc": 0.339, "high school computer science_acc": 0.232, "global facts_acc": 0.354, "clinical knowledge_acc": 0.402, "formal logic_acc": 0.296, "college physics_acc": 0.198, "logical fallacies_acc": 0.377, "marketing_acc": 0.386, "high school world history_acc": 0.436, "philosophy_acc": 0.442, "international law_acc": 0.442, "astronomy_acc": 0.331, "high school mathematics_acc": 0.223, "sociology_acc": 0.545, "nutrition_acc": 0.354, "elementary mathematics_acc": 0.231, "high school psychology_acc": 0.371, "management_acc": 0.304, "abstract algebra_acc": 0.242, "professional medicine_acc": 0.277, "high school us history_acc": 0.429, "high school microeconomics_acc": 0.274, "college mathematics_acc": 0.222, "moral disputes_acc": 0.409, "medical genetics_acc": 0.384, "us foreign policy_acc": 0.505, "virology_acc": 0.382, "high school chemistry_acc": 0.282, "machine learning_acc": 0.279, "professional law_acc": 0.307, "professional accounting_acc": 0.302, "conceptual physics_acc": 0.261, "moral scenarios_acc": 0.239, "college medicine_acc": 0.291, "electrical engineering_acc": 0.271, "college biology_acc": 0.385, "professional psychology_acc": 0.34, "prehistory_acc": 0.396, "high school physics_acc": 0.22, "high school biology_acc": 0.379, "human aging_acc": 0.36, "college chemistry_acc": 0.242, "human sexuality_acc": 0.315, "high school european history_acc": 0.451, "miscellaneous_acc": 0.471, "anatomy_acc": 0.41, "high school statistics_acc": 0.181, "jurisprudence_acc": 0.346, "public relations_acc": 0.312, "security studies_acc": 0.316, "world religions_acc": 0.476, "computer security_acc": 0.384, "econometrics_acc": 0.23, "business ethics_acc": 0.374, "high school geography_acc": 0.355, "high school macroeconomics_acc": 0.311, "high school government and politics_acc": 0.396, "college computer science_acc": 0.313}

% llama-7b + MERIt (ar) step 500 
%{"overall_acc": 0.34, "high school computer science_acc": 0.222, "global facts_acc": 0.354, "clinical knowledge_acc": 0.375, "formal logic_acc": 0.288, "college physics_acc": 0.188, "logical fallacies_acc": 0.358, "marketing_acc": 0.403, "high school world history_acc": 0.445, "philosophy_acc": 0.426, "international law_acc": 0.458, "astronomy_acc": 0.371, "high school mathematics_acc": 0.216, "sociology_acc": 0.54, "nutrition_acc": 0.344, "elementary mathematics_acc": 0.257, "high school psychology_acc": 0.369, "management_acc": 0.304, "abstract algebra_acc": 0.242, "professional medicine_acc": 0.306, "high school us history_acc": 0.438, "high school microeconomics_acc": 0.283, "college mathematics_acc": 0.222, "moral disputes_acc": 0.386, "medical genetics_acc": 0.424, "us foreign policy_acc": 0.515, "virology_acc": 0.376, "high school chemistry_acc": 0.272, "machine learning_acc": 0.306, "professional law_acc": 0.302, "professional accounting_acc": 0.302, "conceptual physics_acc": 0.286, "moral scenarios_acc": 0.238, "college medicine_acc": 0.308, "electrical engineering_acc": 0.257, "college biology_acc": 0.385, "professional psychology_acc": 0.336, "prehistory_acc": 0.396, "high school physics_acc": 0.227, "high school biology_acc": 0.382, "human aging_acc": 0.342, "college chemistry_acc": 0.273, "human sexuality_acc": 0.3, "high school european history_acc": 0.463, "miscellaneous_acc": 0.472, "anatomy_acc": 0.381, "high school statistics_acc": 0.205, "jurisprudence_acc": 0.364, "public relations_acc": 0.303, "security studies_acc": 0.352, "world religions_acc": 0.476, "computer security_acc": 0.404, "econometrics_acc": 0.23, "business ethics_acc": 0.354, "high school geography_acc": 0.325, "high school macroeconomics_acc": 0.319, "high school government and politics_acc": 0.396, "college computer science_acc": 0.313}


% {"overall_acc": 0.415, "high school computer science_acc": 0.404, "global facts_acc": 0.333, "clinical knowledge_acc": 0.439, "formal logic_acc": 0.296, "college physics_acc": 0.158, "logical fallacies_acc": 0.451, "marketing_acc": 0.657, "high school world history_acc": 0.597, "philosophy_acc": 0.506, "international law_acc": 0.608, "astronomy_acc": 0.417, "high school mathematics_acc": 0.216, "sociology_acc": 0.64, "nutrition_acc": 0.39, "elementary mathematics_acc": 0.241, "high school psychology_acc": 0.574, "management_acc": 0.559, "abstract algebra_acc": 0.232, "professional medicine_acc": 0.391, "high school us history_acc": 0.527, "high school microeconomics_acc": 0.371, "college mathematics_acc": 0.222, "moral disputes_acc": 0.449, "medical genetics_acc": 0.455, "us foreign policy_acc": 0.697, "virology_acc": 0.424, "high school chemistry_acc": 0.292, "machine learning_acc": 0.414, "professional law_acc": 0.335, "professional accounting_acc": 0.31, "conceptual physics_acc": 0.432, "moral scenarios_acc": 0.236, "college medicine_acc": 0.39, "electrical engineering_acc": 0.354, "college biology_acc": 0.441, "professional psychology_acc": 0.424, "prehistory_acc": 0.514, "high school physics_acc": 0.207, "high school biology_acc": 0.463, "human aging_acc": 0.428, "college chemistry_acc": 0.263, "human sexuality_acc": 0.469, "high school european history_acc": 0.518, "miscellaneous_acc": 0.601, "anatomy_acc": 0.507, "high school statistics_acc": 0.163, "jurisprudence_acc": 0.57, "public relations_acc": 0.523, "security studies_acc": 0.348, "world religions_acc": 0.635, "computer security_acc": 0.545, "econometrics_acc": 0.248, "business ethics_acc": 0.434, "high school geography_acc": 0.487, "high school macroeconomics_acc": 0.344, "high school government and politics_acc": 0.615, "college computer science_acc": 0.253}

% {"overall_acc": 0.424, "high school computer science_acc": 0.394, "global facts_acc": 0.343, "clinical knowledge_acc": 0.477, "formal logic_acc": 0.304, "college physics_acc": 0.218, "logical fallacies_acc": 0.463, "marketing_acc": 0.691, "high school world history_acc": 0.606, "philosophy_acc": 0.532, "international law_acc": 0.492, "astronomy_acc": 0.437, "high school mathematics_acc": 0.23, "sociology_acc": 0.625, "nutrition_acc": 0.452, "elementary mathematics_acc": 0.228, "high school psychology_acc": 0.592, "management_acc": 0.578, "abstract algebra_acc": 0.232, "professional medicine_acc": 0.461, "high school us history_acc": 0.576, "high school microeconomics_acc": 0.418, "college mathematics_acc": 0.242, "moral disputes_acc": 0.394, "medical genetics_acc": 0.495, "us foreign policy_acc": 0.667, "virology_acc": 0.43, "high school chemistry_acc": 0.327, "machine learning_acc": 0.396, "professional law_acc": 0.345, "professional accounting_acc": 0.317, "conceptual physics_acc": 0.393, "moral scenarios_acc": 0.238, "college medicine_acc": 0.395, "electrical engineering_acc": 0.354, "college biology_acc": 0.413, "professional psychology_acc": 0.406, "prehistory_acc": 0.508, "high school physics_acc": 0.227, "high school biology_acc": 0.495, "human aging_acc": 0.333, "college chemistry_acc": 0.263, "human sexuality_acc": 0.531, "high school european history_acc": 0.567, "miscellaneous_acc": 0.593, "anatomy_acc": 0.485, "high school statistics_acc": 0.209, "jurisprudence_acc": 0.523, "public relations_acc": 0.495, "security studies_acc": 0.471, "world religions_acc": 0.582, "computer security_acc": 0.515, "econometrics_acc": 0.212, "business ethics_acc": 0.455, "high school geography_acc": 0.508, "high school macroeconomics_acc": 0.404, "high school government and politics_acc": 0.63, "college computer science_acc": 0.283}  % step 100

\begin{table*}[t]
\centering
\setlength{\tabcolsep}{2.5mm}{
\scalebox{0.8}{
\begin{tabular}{lcccc}
\hline
\textbf{Category}               & \textbf{\llama-7B} & \textbf{\llama-7B + \meritp} & \textbf{\llama-13B} & \textbf{\llama-13B + \meritp} \\
\hline
High School Computer Science    & 26.3          & 23.2      & 40.4      & 39.4\\
Global Facts                    & 29.3          & \bf{35.4} & 33.3      & \textbf{34.3}\\
Clinical Knowledge              & 36.7          & \bf{40.2} & 43.9      & \textbf{47.7}\\
Formal Logic                    & 30.4          & 29.6      & 29.6      & \textbf{30.4}\\
College Physics                 & 17.8          & \bf{19.8} & 15.8      & \textbf{21.8}\\
Logical Fallacies               & 40.1          & 37.7      & 45.1      & \textbf{46.3}\\
Marketing                       & 36.5          & \bf{38.6} & 65.7      & \textbf{69.1}\\
High School World History       & 37.7          & \bf{43.6} & 59.7      & \textbf{60.6}\\
Philosophy                      & 39.0          & \bf{44.2} & 50.6      & \textbf{53.2}\\
International Law               & 49.2          & 44.2      & 60.8      & 49.2\\
Astronomy                       & 31.1          & \bf{33.1} & 41.7      & \textbf{43.7}\\
High School Mathematics         & 20.8          & \bf{22.3} & 21.6      & \textbf{23.0}\\
Sociology                       & 42.5          & \bf{54.5} & 64.0      & 62.5\\
Nutrition                       & 32.8          & \bf{35.4} & 39.0      & \textbf{45.2}\\
Elementary Mathematics          & 21.5          & \bf{23.1} & 24.1      & 22.8\\
High School Psychology          & 31.2          & \textbf{37.1}      & 57.4      & \textbf{59.2}\\ 
Management                      & 30.4          & 30.4      & 55.9      & \textbf{57.8}\\
Abstract Algebra                & 22.2          & \textbf{23.1}      & 23.2      & 23.2\\
Professional Medicine           & 23.6          & \textbf{27.7}      & 39.1      & \textbf{46.1}\\
High School US History          & 41.4          & \textbf{42.9}      & 52.7      & \textbf{57.6}\\
High School Microeconomics      & 27.8          & \textbf{28.2}      & 37.1      & \textbf{41.8}\\
College Mathematics             & 23.2          & 22.2      & 22.2      & \textbf{24.2}\\
Moral Disputes                  & 23.8          & \textbf{40.9}      & 44.9      & 39.4\\
Medical Genetics                & 37.4          & \textbf{38.4}     & 45.5      & \textbf{49.5}\\
US Foreign Policy               & 39.4          & \textbf{51.5}      & 69.7      & 66.7\\
Virology                        & 30.9          & \textbf{37.6}      & 42.4      & \textbf{43.0}\\
High School Chemistry           & 24.8          & \textbf{27.2}      & 29.2      & \textbf{32.7}\\
Machine Learning                & 31.5          & 30.6      & 41.4      & 39.6\\
Professional Law                & 28.9          & \textbf{30.2}      & 33.5      & \textbf{34.5}\\
Professional Accounting         & 30.6          & 30.2      & 31.0      & \textbf{31.7}\\
Conceptual Physics              & 28.2          & \textbf{28.6}      & 43.2      & 39.3\\
Moral Scenarios                 & 23.8          & 23.8      & 23.6      & 23.8\\
College Medicine                & 29.1          & \textbf{30.8}      & 39.0      & \textbf{39.5}\\
Electrical Engineering          & 25.0          & \textbf{25.7}      & 35.4      & 35.4\\
College Biology                 & 33.6          & \textbf{38.5}      & 44.1      & 41.3\\
Professional Psychology         & 33.9          & 33.6      & 42.4      & 40.6\\
Prehistory                      & 38.1          & \textbf{39.6}      & 26.3      & \textbf{50.8}\\
High School Physics             & 18.0          & \textbf{22.7}      & 20.7      & \textbf{22.7}\\
High School Biology             & 34.0          & \textbf{38.2}      & 46.3      & \textbf{49.5}\\
Human Aging                     & 31.1          & \textbf{34.2}      & 42.8      & 33.3\\
College Chemistry               & 19.2          & \textbf{27.3}      & 26.3      & 26.3\\
Human Sexuality                 & 31.5          & 30.0      & 46.9      & \textbf{53.1}\\
High School European History    & 37.2          & \textbf{46.3}      & 51.8      & \textbf{56.7}\\
Miscellaneous                   & 38.6          & \textbf{47.2}      & 60.1      & 59.3\\
Anatomy                         & 38.1          & 38.1      & 50.7      & 48.5\\
High School Statistics          & 15.8          & \textbf{20.5}      & 48.7      & 20.9\\
Jurisprudence                   & 28.0          & \textbf{36.4}      & 57.0      & 52.3\\
Public Relations                & 26.6          & \textbf{30.3}      & 52.3      & 49.5\\
Security Studies                & 23.0          & \textbf{35.2}      & 34.8      & \textbf{47.1}\\
World Religions                 & 43.5          & \textbf{47.6}      & 63.5      & 58.2\\
Computer Security               & 29.3          & \textbf{40.4}      & 54.5      & 51.5\\
Econometrics                    & 23.9          & 23.0      & 24.8      & 21.2\\
Business Ethics                 & 41.4          & 35.4      & 43.4      & \textbf{45.5}\\
High School Geography           & 29.9          & \textbf{32.5}      & 48.7      & \textbf{50.8}\\
High School Macroeconomics      & 27.2          & \textbf{31.9}      & 34.4      & \textbf{40.4}\\
High School Government and Politics & 34.9      & \textbf{39.6}      & 61.5      & \textbf{63.0}\\
College Computer Science        & 27.3          & \textbf{31.3}      & 25.3      & \textbf{28.3}\\ \hline
Average                         & 30.9          & \textbf{34.0}      & 41.5      & \textbf{42.4}\\          
\hline
\end{tabular}
}}
\caption{Sub-task accuracy of MMLU. Better results are highlighted in bold.}
\label{tab:mmlu-detail}
\end{table*}

==> tables/race.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4.0mm}{
\scalebox{0.9}{
\begin{tabular}{lccccccc}
% \hline
\toprule
Model / Dataset              & Dev       & Test       \\ \hline
\llama-7B                    & 34.9      & 36.0      \\
~~~~w/ \meritp                & \bf{39.5} & \bf{39.7}      \\ % 100 step
%%~~~~w/ \merit~(ctr)       & \bf{31.2}   & \bf{31.1}   & \bf{29.2}        & \bf{29.6}   & \bf{53.0}& \bf{52.4} \\ % 500 step \hline  %save for next version 2023-05-20 
\hdashline
\llama-13B                   & 56.8      & 56.2      \\
~~~~w/ \meritp                & \bf{57.4} & \bf{57.0} \\ % 100step for zero-shot and 500 step for 5-shot MMLU 
\hdashline
\llama-33B                   & 64.3 & 62.9  \\
~~~~w/ \lora{\meritp}        & \bf{68.9} & \bf{67.5}  \\ % 100 step 
% \hdashline
\bottomrule
\end{tabular}
}}
% \caption{The results of \llama~series models on RACE and MMLU. $^\dag$ means the results are reported in the Open LLM Leaderboard. \teng{46.9 of LLaMA-13B on MMLU reported by FranxYao https://github.com/FranxYao/chain-of-thought-hub/tree/main}.}
\caption{The results of \llama~series models on RACE benchmark.}
\vspace{-0.3cm}
\label{tab:race}
\end{table}
